Safety-Aware Preference-Based Learning for Safety-Critical Control

Bringing dynamic robots into the wild requires a tenuous balance between performance and safety. Yet controllers designed to provide robust safety guarantees often result in conservative behavior, and tuning these controllers to find the ideal trade-off between performance and safety typically requires domain expertise or a carefully constructed reward function. This work presents a design paradigm for systematically achieving behaviors that balance performance and robust safety by integrating safety-aware Preference-Based Learning (PBL) with Control Barrier Functions (CBFs). Fusing these concepts -- safety-aware learning and safety-critical control -- gives a robust means to achieve safe behaviors on complex robotic systems in practice. We demonstrate the capability of this design paradigm to achieve safe and performant perception-based autonomous operation of a quadrupedal robot both in simulation and experimentally on hardware.

==> Sections/AT_SecIII_Draft.tex <==
In this section we formalize robust safety and discuss safe controller synthesis through the use of Control Barrier Functions (CBFs).
Consider the following nonlinear control-affine system:
\begin{equation}
    \dot{\mb{x}} = \mb{f}(\mb{x}) + \mb{g}(\mb{x})\mb{v},
    \label{eq:reduced_model}
\end{equation}
with state ${\mb{x} \in \R^{n}}$,
input ${\mb{v} \in \R^{m}}$, and functions ${\mb{f}:\R^{n}\to\R^{n}}$ and ${\mb{g} : \R^{n}\to\R^{n \times m}}$ assumed to be locally Lipschitz continuous on their domains. Specifying the input via a state-feedback controller $\mb{k}:\R^{n}\to \R^{m}$ that is locally Lipschitz continuous on its domain yields the closed-loop system:
\begin{equation}
    \dot{\mb{x}} = \mb{f}(\mb{x}) + \mb{g}(\mb{x})\mb{k}(\mb{x}).
    \label{eq:closed_loop_system}
\end{equation}
We assume that for any initial condition ${\mb{x}(0) = \mb{x}_0 \in \R^{n}}$, this system has a unique solution $\mb{x}(t)$ that exists for all $t \in \R_{\geq 0}$. Let a set $\mathcal{C} \subset \R^{n}$, referred to as the \textit{safe set}, be defined as the 0-superlevel set of a continuously differentiable function $h:\R^{n}\times\R^p\to\R$: 
\begin{equation}
    \mathcal{C} = \{ \mb{x} \in \R^{n} : h(\mb{x},\bs{\rho}) \geq 0 \}, \label{eq:safe_set}
\end{equation}
where the constant $\bs{\rho}\in\R^p$ is a set of parameters. We formally define safety as follows:
\begin{definition}[Forward Invariance and Safety \citep{ames2017control}] \label{def:CBF}
     The set $\mathcal{C} \subset \R^{n}$ is forward invariant if for every $\mb{x}_0 \in \mathcal{C}$ the solution $\mb{x}(t)$ to \eqref{eq:closed_loop_system} satisfies $\mb{x}(t) \in \mathcal{C}$ for all $t \geq 0 $. The system \eqref{eq:closed_loop_system} is safe with respect to $\mathcal{C}$ if $\mathcal{C}$ is forward invariant. 
\end{definition}

The parameter $\bs{\rho}\in\R^p$ often contains information about the system's environment that designates a given state as safe or unsafe, such as the location and size of obstacles. In highly unstructured environments the system may need to form an estimate of $\bs{\rho}$, denoted by $\widehat{\bs{\rho}}\in\R^p$ from measurements of the environment, such as image data. It is frequently the case that the process of converting complex measurements such as images into the low-dimensional representation $\widehat{\bs{\rho}}$ is imperfect, leading to an error between the estimator $\widehat{\bs{\rho}}$ and the true value of $\bs{\rho}$. In this setting, safety-critical control can be achieved via Measurement-Robust Control Barrier Functions (MR-CBFs):
\begin{definition}[Measurement-Robust Control Barrier Functions \citep{dean2020guaranteeing}]
The function $h$ is a \textit{Measurement-Robust Control Barrier Function} (MR-CBF) for \eqref{eq:reduced_model} on $\C$ with parameters $a,b\in\R_{\geq 0}$ if there exists $\alpha\in\mathcal{K}_\infty^{e}$\footnote{We say that a continuous function ${\alpha : \R_{\geq 0} \to \R_{\geq 0}}$ is {\em class~$\mathcal{K}_\infty$} (${\alpha \in \mathcal{K}_\infty}$) if ${\alpha(0) = 0}$, $\alpha$ is strictly monotonically increasing, and $\lim_{r\to\infty}\alpha(r) = \infty$. We say that a continuous function $\alpha : \R \to \R$ is {\em class~$\mathcal{K}^{e}_\infty$} (${\alpha \in \mathcal{K}^e_{\infty}}$) if ${\alpha(0) = 0}$, $\alpha$ is strictly monotonically increasing, $\lim_{r\to\infty}\alpha(r) = \infty$, and $\lim_{r\to-\infty}\alpha(r) = -\infty$.} such that for all $\widehat{\bs{\rho}}\in\R^p$ and $\mb{x}\in\R^n$:
\begin{equation} 
    \label{eq:mr_cbf_constraint}
        \sup_{\mb{v} \in \R^{m}}
        \underbrace{\derp{h}{\mb{x}}(\mb{x},\widehat{\bs{\rho}})\mb{f}(\mb{x})}_{L_\mb{f}h(\mb{x},\widehat{\bs{\rho}})} + \underbrace{\derp{h}{\mb{x}}(\mb{x},\widehat{\bs{\rho}})\mb{g}(\mb{x})}_{L_\mb{g}h(\mb{x},\widehat{\bs{\rho}})}\mb{v} - a - b\Vert\mb{v}\Vert> -\alpha(h(\mb{x},\widehat{\bs{\rho}})), 
\end{equation}
\end{definition}
\begin{theorem}[\cite{dean2020guaranteeing}] \label{thm:mrcbf}
Suppose the functions $L_\mb{f}h$, $L_\mb{g}h$, and $\alpha\circ h$ are Lipschitz continuous on $\R^n\times\R^p$. If $\Vert\widehat{\bs{\rho}}-\bs{\rho}\Vert \leq \epsilon$ for some $\epsilon\in\R_{\geq 0}$, then there exists $\underline{a},\underline{b}\in\R_{\geq 0}$ such that for any $a,b\in\R_{\geq 0}$ satisfying $a\geq\underline{a}$ and $b\geq\underline{b}$ and locally Lipschitz continuous controller $\mb{k}:\R^n\to\R^m$ satisfying:
 \begin{equation} \label{eq:mr_constraint}
        L_\mb{f}h(\mb{x},\widehat{\bs{\rho}}) + L_\mb{g}h(\mb{x},\widehat{\bs{\rho}})\mb{k}(\mb{x}) + a + b\Vert\mb{k}(\mb{x})\Vert \geq -\alpha(h(\mb{x},\widehat{\bs{\rho}})),
    \end{equation}
for all $\mb{x}\in\R^n$, the system \eqref{eq:closed_loop_system} is safe with respect to $\C$.    
\end{theorem}

An additional challenge frequently encountered when deploying model-based controllers onto real-world systems is a mismatch between the commanded input and the input actually received by the system, captured by the disturbed open-loop system:
\begin{equation}
    \dot{\mb{x}} = \mb{f}(\mb{x}) + \mb{g}(\mb{x}) (\mb{v}+\mb{d}(t)),
    \label{eq:reduced_model_dist}
\end{equation}
with a piecewise continuous disturbance signal ${\mb{d}(t):\R_{\geq 0} \to \R^{m}}$ for which we define $\Vert\mb{d}\Vert_{\infty} \triangleq \sup_{t \geq 0} \Vert\mb{d}\Vert$. A locally Lipschitz continuous controller $\mb{k}:\R^n\to\R^m$ yields closed-loop dynamics:
\begin{equation}
    \dot{\mb{x}} = \mb{f}(\mb{x}) + \mb{g}(\mb{x}) (\mb{k}(\mb{x})+\mb{d}(t)),
    \label{eq:closed_loop_dist}
\end{equation}
While it may possible to synthesize controllers that render a given set $\C$ safe in the presence of disturbances \citep{jankovic2018robust}, this may result in overly-conservative behavior. Instead, we consider how safety properties degrade with disturbances via the following definition:

\begin{definition}[Input-to-State Safety (ISSf) \citep{kolathaya2018input}]
\label{def:issf}
   The system \eqref{eq:closed_loop_dist} is input-to-state safe with respect to $\mathcal{C}$ if there exists $\gamma \in \mathcal{K}$ such that for all $\delta\in\R_{\geq 0}$ and $\mb{d}:\R_{\geq 0}\to\R^m$ satisfying $\Vert\mb{d}\Vert_\infty\leq\delta$, the set $\mathcal{C}_{\delta}\subset\R^n$ defined as: 
    \begin{align}
       \mathcal{C}_{\delta} = \{\mb{x} \in \R^{n} : h(\mb{x}, \bs{\rho}) \geq - \gamma(\delta)\},
    \end{align}
    is forward invariant.
\end{definition}
This definition requires that in the absence of disturbances ($\delta = 0$), the original set $\C$ is safe. In the presence of disturbances, a neighborhood of $\C$ is safe, rather than $\C$ itself. Given this definition, ISSf Control Barrier Functions (ISSf-CBFs) can be used to design controllers that ensure \eqref{eq:closed_loop_dist} is input-to-state safe with respect to $\mathcal{C}$ and which regulate the size of the set $\mathcal{C}_{\delta}$:
\begin{definition}[Input-to-State Safe Control Barrier Function (ISSf-CBF) \citep{alan2021safe}]
    The function $h$ is an Input-to-State Safe Control Barrier Function (ISSf-CBF) for~(\ref{eq:reduced_model_dist}) on $\C$ with parameter $\sigma\in\R_{\geq 0}$ if there exists $\alpha\in\K_\infty^e$ such that for all $\mb{x} \in \R^{n}$: 
    \begin{equation} \label{eq:issf_cbf_constraint}
        \sup_{\mb{v} \in \R^{m}}
       L_\mb{f}h(\mb{x},\bs{\rho}) + L_\mb{g}h(\mb{x},\bs{\rho})\mb{v}-\sigma\Vert L_\mb{g}h(\mb{x},\bs{\rho}) \Vert^2 > -\alpha(h(\mb{x},\bs{\rho})), 
    \end{equation}
\end{definition}
\begin{theorem}[\cite{alan2021safe}]\label{thm:issf-cbf}
For any locally Lipschitz continuous controller $\mb{k}: \R^{n} \to \R^{m}$ satisfying:
    \begin{equation} \label{eq:issf_constraint}
        L_\mb{f}h(\mb{x},\bs{\rho}) + L_\mb{g}h(\mb{x},\bs{\rho})\mb{k}(\mb{x}) \geq -\alpha(h(\mb{x},\bs{\rho})) + \sigma \Vert L_\mb{g}h(\mb{x},\bs{\rho}) \Vert^2,
    \end{equation}
   for all $\mb{x} \in \R^{n}$, the system \eqref{eq:closed_loop_dist} is ISSf with respect to $\mathcal{C}$ with
    $\gamma(\delta) = -\alpha^{-1}(-\delta^2/4\sigma)$ and $\alpha^{-1}\in\K_\infty^e$. 
\end{theorem}

A setting in which disturbances in the input often arise is when a control system is designed as a set of interconnected subsystems, where the output of one subsystem serves as an input to another subsystem. Many real-life engineering systems have high-dimensional state spaces and complex dynamics for which the problem of control design is separated into the design of a low-dimensional system that provides reference signals capturing safe behavior, and design for a high-dimensional system that tracks these reference signals. In particular, consider the the following cascaded nonlinear control-affine system yielded through the modification of \eqref{eq:reduced_model}:
\begin{equation}
    \dot{\mb{x}} = \mb{f}(\mb{x})+\mb{g}(\mb{x})\bs{\kappa}(\bs{\xi}), \qquad
 \dot{\bs{\xi}} = \mb{f}_{\bs{\xi}}(\mb{x},\bs{\xi}) + \mb{g}_{\bs{\xi}}(\mb{x},\bs{\xi})\mb{u},
 \label{eq:full_system}
\end{equation}
with additional states $\bs{\xi}\in\R^k$, control input $\mb{u} \in \R^l$ and functions
$\bs{\kappa}: \R^k \to \R^m$, $\mb{f}_{\bs{\xi}}:\R^n \times \R^k \to \R^k$, and
$\mb{g}_{\bs{\xi}}:\R^n \times \R^k \to \R^{k \times l}$ assumed to be locally Lipschitz continuous on their domains. We note that the input $\mb{v}$ was replaced by the term $\bs{\kappa}(\bs{\xi})$. These dynamics may represent systems described by the Euler-Lagrange equations, such as mobile robotic systems, where $\mb{x}$ reflects floating-base position coordinates, $\bs{\xi}$ captures both floating-base velocities and individual joint position and velocity coordinates. and the input $\mb{u}$ reflects forces and torques applied to the system. 

Given this cascaded control system, we make two assumptions. First, we assume the safe set $\C$ can be described as in \eqref{eq:safe_set}, such that it is only dependent on the states $\mb{x}$ and parameters $\bs{\rho}$, and does not explicitly depend on the states $\bs{\xi}$. For example, in the context of a mobile robotic system, this assumption is justified if safety is described as keeping the floating base position of the robot away from obstacles. Second, we  assume that there exists a feedback controller $\bs{\pi}:\R^n\times\R^k\times\R^m\to\R^l$ and $\delta\in\R_{\geq 0}$ such that for any continuous, bounded signal $\mb{s}:\R_{\geq 0}\to\R^m$, the closed-loop system:
\begin{equation}
    \dot{\bs{\xi}} = \mb{f}_{\bs{\xi}}(\mb{x},\bs{\xi}) + \mb{g}_{\bs{\xi}}(\mb{x},\bs{\xi})\bs{\pi}(\mb{x},\bs{\xi},\mb{s}(t))
\end{equation}
satisfies the following implication:
\begin{equation}
    \Vert \bs{\kappa}(\bs{\xi}(0)) - \mb{s}(0) \Vert \leq \delta \implies \Vert \bs{\kappa}(\bs{\xi}(t)) - \mb{s}(t) \Vert \leq \delta,\quad t\in\R_{\geq 0}.
\end{equation}
This assumption reflects that a separate controller may be designed for the high-dimensional dynamics of the system that tracks sufficiently well-behaved reference signals synthesized via the low-dimensional model up to some error threshold. In particular, if a controller $\mb{k}:\R^n\to\R^m$ is designed for the low-dimensional system \eqref{eq:reduced_model} and $\Vert\bs{\kappa}(\bs{\xi}(0))-\mb{k}(\mb{x}(0)) \Vert \leq \delta$, then we have that the controller $\bs{\pi}$ ensures $\Vert\bs{\kappa}(\bs{\xi}(t))-\mb{k}(\mb{x}(t))\Vert \leq \delta$ for $t\in\R_{\geq 0}$. In studying the ISSf behavior of \eqref{eq:closed_loop_dist}, the disturbance may be defined as $\mb{d}(t) = \bs{\kappa}(\bs{\xi}(t))-\mb{k}(\mb{x}(t))$, and satisfies $\Vert\mb{d}\Vert_\infty \leq \delta$.
\begin{equation}
    \dot{\mb{x}} = \mb{f}(\mb{x})+\mb{g}(\mb{x})\bs{\kappa}(\bs{\xi}), \qquad
 \dot{\bs{\xi}} = \mb{f}_{\bs{\xi}}(\mb{x},\bs{\xi}) + \mb{g}_{\bs{\xi}}(\mb{x},\bs{\xi})\bs{\pi}(\mb{x},\bs{\xi},\mb{k}(\mb{x})),
%  \label{eq:full_system}
\end{equation}

==> Sections/Appendices/lemmaProof.tex <==
\label{apdx:lemma_proof}

In this appendix we present the proof of Lemma \ref{lem:safety_reduced_model} which establishes the input-to-state safety of $\mathcal{S}$. Recall that Lemma \ref{lem:safety_reduced_model} is given as: 

\begin{lemma*} 
\textit{
Consider system~(\ref{eq:full_system}), velocity $\mb{v}$ satisfying~(\ref{eq:desired_velocity_ISSf}), tracking error $\bs{\eta}$ given by~(\ref{eq:tracking_error}), and a tracking controller $\mb{u}=\Theta(\mb{x},\bs{\xi})$ satisfying Assumption \ref{assp:ISS-tracking}.
Then, $\mathcal{S}$ as defined in \eqref{eq:safe_set_ro} is ISSf, associated with the following forward invariant set:
\begin{equation}
    \mathcal{S}_{\bs{\eta}} = \left\{ (\mb{x},\bs{\xi}) \in \R^n \times \R^k : h_R(\mb{x}, \bs{\rho}) \geq  - \frac{1}{4ab}\overline{\eta}^2 \right\}.
    % \label{eq:invariant_set}
\end{equation}
} 
\end{lemma*}
\noindent
\begin{proof}
\begin{align}
    \dot{h}_R(\mb{x}, \rho) & = \frac{\partial h }{\partial \mb{x}}(\mb{f}(\mb{x}) + \mb{g}(\mb{x})(\mb{v}_d + \eta))  \\
    & \geq -a h(\mb{x}, \rho) + b \left\Vert \frac{\partial h_R}{\partial \mb{x}}\mb{g}(\mb{x})  \right\Vert^2 - \left\Vert \frac{\partial h_R}{\partial \mb{x}}\mb{g}(\mb{x}) \right\Vert \left \Vert \eta \right\Vert\\
    & \geq - ah_R(\mb{x}, \rho) +   \left(\sqrt{b}\Vert \frac{\partial h_R}{\partial \mb{x}} \mb{g}(\mb{x}) \Vert - \frac{1}{2 \sqrt{b} } \Vert \eta \Vert \right)^2 - \frac{1}{4b}\Vert \eta \Vert^2 \\
    & \geq - a h(\mb{x}, \rho) - \frac{1}{4b} \overline{\eta}^2. 
\end{align}
So 
\begin{equation}
    h(\mb{x}, \rho)+ \frac{1}{4ab}\overline{\eta}^2 \leq 0 \implies \dot{h}_R \geq 0 
\end{equation}
which also implies that $\frac{d}{dt}(h_R + \frac{1}{4ab}\Vert \overline{\eta} \Vert^2) \geq 0 $ for all $h(\mb{x}, \rho) + \frac{1}{4ab}\Vert \overline{\eta}\Vert^2 = 0 $, so the set $\mathcal{S}_{e,\mb{d}}$ is invariant with the class $\mathcal{K}$ function $\iota(\overline\eta) = \frac{1}{4ab}\overline{\eta}^2$ by Nagumo's theorem \cite{nagumo1942lage} and thus the set $\mathcal{S}$ is ISSf by defition. 
\end{proof}

% \textcolor{red}{
% \begin{proof}
% % Let us pick $\sigma$ such that:
% % \begin{equation}
% %     \sigma \geq \frac{\alpha_{\rm e}}{4(k_{3} - k_{2} \alpha)},
% %     \label{eq:sigma_condition}
% % \end{equation}
% % and let us define ${h_{V,d} : \mathcal{Z} \to \R}$
% Let us define ${h_{V,d} : \mathcal{Z} \times \R^p \to \R}$:
% \begin{equation}
%     h_{V,d}(z,\rho) = - V(\eta) + \alpha_{\rm e} h(x,\rho) + \frac{1}{\alpha} \iota(\| d \|_{\infty}).
%     \label{eq:extended_barrier}
% \end{equation}
% % Then, ${\mathcal{S}_{V} = \{ z \in \mathcal{Z} : h_{V}(z) \geq 0 \}}$.
% % Notice that if ${\| d \|_{\infty} = 0}$, ${h_{V}(z) \geq 0 \Rightarrow h(x) \geq 0}$ since ${V(\eta) \geq 0}$, i.e., we have ${\mathcal{S}_{V} \subset S}$.
% To show the invariance of $\mathcal{S}_{V,d}$, we apply Theorem \ref{thm:CBF} and prove that ${\dot{h}_{V,d}(z,\rho,k(z)) \geq - \alpha h_{V,d}(z,\rho)}$ as follows:
% % \begin{align}
% % \begin{split}
% %     \dot{h}_{V,d} & (z,k(z)) + \alpha h_{V,d}(z) \\
% %     & = - \dot{V}(z,k(z)) + \alpha_{\rm e} \frac{\partial h(x)}{\partial x} (f(x) + g(x) (v_{\rm d} + \eta)) - \alpha V(\eta) + \alpha \alpha_{\rm e} h(x) + \iota(\| d \|_{\infty}) \\
% %     & \geq k_{3} \| \eta \|^2 + \alpha_{\rm e} \sigma \left\| \frac{\partial h(x)}{\partial x} g(x) \right\|^2 - \alpha_{\rm e} \left\| \frac{\partial h(x)}{\partial x} g(x) \right\| \| \eta \| - \alpha k_{2} \| \eta \|^2 \\
% %     & \geq (k_{3} - k_{2} \alpha) \| \eta \|^2 + \left( \sqrt{\alpha_{\rm e} \sigma} \left\| \frac{\partial h(x)}{\partial x} g(x) \right\| - \frac{\sqrt{\alpha_{\rm e}}}{2 \sqrt{\sigma}} \| \eta \| \right)^2 - \frac{\alpha_{\rm e}}{4 \sigma} \| \eta \|^2 \\
% %     & \geq \left( k_{3} - k_{2} \alpha - \frac{\alpha_{\rm e}}{4 \sigma} \right)  \| \eta \|^2 \geq 0.
% % \end{split}
% % \end{align}
% % In the four lines of the inequality we used:
% % (\ref{eq:extended_barrier}) and~(\ref{eq:reduced_model});
% % (\ref{eq:tracking_controller_ISS}),~(\ref{eq:desired_velocity_ISSf}) and the Cauchy-Schwartz inequality;
% \begin{align}
% \begin{split}
%     \dot{h}_{V,d} & (z,\rho,\Theta(z)) 
%     = - \dot{V}(z,\Theta(z)) + \alpha_{\rm e}(L_fh(x,\rho) + L_gh(x,\rho) (v_{\rm d} + \eta)) \\
%     & \geq k_3 \Vert \eta \Vert^2 - \iota(\Vert d \Vert_\infty) - \alpha_{\rm e}\alpha h(x,\rho) + \alpha_{\rm e}\sigma \Vert L_gh(x,\rho)\Vert^2 - \alpha_{\rm e}\Vert L_gh(x,\rho)\Vert \Vert \eta \Vert \\
%     & \geq (k_3-k_2\alpha) \Vert \eta \Vert^2 - \alpha h_{V,d}(z,\rho) + \alpha_{\rm e} \left(\sqrt{\sigma}\Vert L_gh(x,\rho)\Vert-\frac{1}{2\sqrt{\sigma}}\Vert\eta\Vert \right)^2 -  \frac{\alpha_{\rm e}}{4\sigma}\Vert\eta\Vert^2 \\
%     & \geq (k_3-k_2\alpha-\frac{\alpha_{\rm e}}{4\sigma}) \Vert \eta \Vert^2 - \alpha h_{V,d}(z,\rho) \\
%     & \geq -\alpha h_{V,d}(z,\rho)
% \end{split}
% \end{align}
% In the four lines of the inequality we used:
% (\ref{eq:tracking_controller_ISS}),~(\ref{eq:desired_velocity_ISSf}) and the Cauchy-Schwartz inequality; adding and subtracting terms $\alpha V(\eta)$ and $\frac{\alpha_{\rm e}}{4\sigma}\Vert\eta\Vert^2$, the upper bound on $V$ in (\ref{eq:tracking_controller_ISS}) and definition \eqref{eq:extended_barrier};
% and finally the condition on $\sigma$ given as $\sigma \geq \frac{\alpha_{\rm e}}{4(k_{3} - k_{2} \alpha)}$. 
% Since $\mathcal{S}_{V,d}$ is forward invariant and $\frac{1}{\alpha_e\alpha} \iota \in \mathcal{K}$, it follows by definition that $\mathcal{S}_V$ is ISSf. 
% % Additionally, since $V$ is positive definite, it follows that: 
% % \begin{align}
% %     h(x) \geq \frac{1}{\alpha_e} \left( V(\eta) - \frac{1}{\alpha} \iota(\Vert d\Vert_\infty) \right) \\
% %     \geq- \frac{1}{\alpha_e\alpha }  \iota(\Vert d\Vert_\infty).
% % \end{align}
% % Let $\mathcal{S}_d = \{z \in \R^n : h(x) \geq - \frac{1}{\alpha_e\alpha}\iota(\Vert d \Vert_\infty )  \} $. Since $\mathcal{S}_d \supset \mathcal{S}_V$, the invariance of $\mathcal{S}_V$ implies the invariance of $\mathcal{S}_d$. Therefore $\mathcal{S}$ is input-to-state safe. 
% \end{proof}
% }



==> Sections/Appendices/pblAppdx.tex <==

We model the posterior as proportional to the product of likelihood and the prior:
\begin{align*}
    \P(\util \mid \data) \propto \P(\data \mid \util)\P(\util),
\end{align*}
where we define the Gaussian prior over $\util$ as:
\begin{align*}
    \P(\util) = \frac{1}{(2\pi)^{\frac{|\act|}{2}} | \Sigma^{\textrm{pr}}| ^{\frac{1}{2}}} \exp \left( -\frac{1}{2}\util^{T}(\Sigma^{\textrm{pr}})^{-1} \util \right),
\end{align*}
with $\Sigma^{\textrm{pr}} \in \R^{|\act| \times |\act|}$ being a prior covariance matrix with each element $[\Sigma^{\textrm{pr}}_{ij}] = \mathcal{K}(\act_i,\act_j)$ and any kernel $\mathcal{K}$. In this work, we use a squared exponential kernel:
\begin{align*}
    \mathcal{K}_{\text{SE}}(\act,\act') = \sigma^2 \exp\left( - \frac{(\act - \act')^2}{2\mb{l}^2} \right) + \varepsilon,
\end{align*} 
where $\sigma \in \R$ is the output variance hyperparameter, $\mb{l} \in \R^d$ is a vector of lengthscales for each dimension of $\act$, and $\varepsilon$ is a kernel noise hyperparameter. The output variance $\sigma$ dictates the expected amplitude of the underlying function. The lengthscales $l_i$, $i \in \{1,\dots,d\}$, are hyperparameters that dictate the expected maximum amount that the underlying function varies in each dimension (the ``wiggliness'').


% \section{Andrew's Dynamics}
% \textcolor{red}{
% Consider the following nonlinear control-affine cascaded system:
% \begin{align}
%     \dot{\mb{x}} &= \mb{f}(\mb{x})+\mb{g}(\mb{x})\bs{\kappa}(\bs{\xi}) \\ \dot{\bs{\xi}} &= \mb{f}_{\bs{\xi}}(\mb{x},\bs{\xi}) + \mb{g}_{\bs{\xi}}(\mb{x},\bs{\xi})\mb{u}
% \end{align}
% with states $\mb{x},\bs{\xi}\in\R^n$, input $\mb{u}\in\R^m$, and functions $\mb{f}:\R^n\to\R^n$, $\mb{g}:\R^n\to\R^{n\times n}$, $\mb{f}_{\bs{\xi}}:\R^n\times\R^n\to\R^n$, and  $\mb{g}_{\bs{\xi}}:\R^n\times\R^n\to\R^{n\times m}$ assumed to be locally Lipschitz continuous on their domains. These dynamics may represent systems described by the Euler-Lagrange equations, such as robotic systems, where $\mb{x}$ and $\bs{\xi}$ reflect the position and velocity coordinates, respectively, and the input $\mb{u}$ reflects forces and torques applied to the system. 
% Motivated by \cite{molnar2021model}, this cascaded model is taken for two reasons.
% The first reason is that the dynamics of the state $\bs{\xi}$ may often be very complicated, such as in the case of legged locomotion \AT{CITE}.
% It is often the case that the control of these dynamics is treated as a separate subsystem, 
% The second reason is that many safety requirements (such as collision-avoidance) are specified as constraints on the position, or the state $\mb{x}$, rather than on both states $\mb{x}$ and $\bs{\xi}$. 
% There exists $\mb{k}:\R^{n?}\to\R^m$ such that:
% \begin{equation}
%     \Vert \bs{\xi}-\bs{\xi}_d(t)\Vert \leq \epsilon
% \end{equation}
% }

==> Sections/ISS.tex <==

An important notion of stability in the case of bounded disturbances is input-to-state stability (ISS). In this work we will consider exponential input-to-state stability. 

\begin{definition}[Input-to-State Stability (ISS) \citep{sontag2008input}]
\label{def:iss}
    The system~(\ref{eq:full_system}) is exponentially input-to-state stable to the origin ${z=0}$ if there exist ${\gamma, M, \beta \in \mathbb{R}_{>0}}$ and ${\mu \in \mathcal{K}}$ such that \begin{equation}
        % \| z_{0} \| \leq \gamma \Rightarrow 
        \| z(t) \| \leq M {\rm e}^{-\beta t} \| z_{0} \| + \mu(\| d \|_{\infty}), \quad \forall t \geq 0. \label{eq:ISS}
    \end{equation}
\end{definition}
An ISS system is stable to the origin if the disturbance is uniformly zero ($d \equiv 0 $) and it is stable to a neighborhood of the origin if $\Vert d \Vert_\infty  > 0 $.
% ISS can be certified by Lyapunov functions as follows.

% \begin{theorem}[\cite{sontag2008input}]
% The system \eqref{eq:full_system} is exponentially input-to-state stable for $d: \R_{\geq 0}\to \mathcal{D}$ if there exists a continuously differentiable function $V: \mathcal{Z} \to \R_{\geq 0}$, parameters $k_1, k_2, k_3 \in \R_{>0}$, and $\iota \in \mathcal{K}$ such that for all $z \in \mathcal{Z}$: 
% \begin{align}
%     \begin{split}
%         k_{1} \| z \|^2&  \leq V(z) \leq k_{2} \| z \|^2, \\
%         \dot{V}(z,k(z)) &  \leq -  k_{3} \| z \|^2 + \iota (\|d\|_{\infty}).
%     \end{split}
%     \label{def:ISS}
% \end{align}
% where ${\dot{V}(z,k(z)) = \frac{\partial V(z)}{\partial z} (F(z) + G(z) (k(z)+d))}$ is the derivative of $V$ along~\eqref{eq:full_system}.
% \end{theorem}



==> Sections/ISSf.tex <==
We formalize the notion of safety as the forward invariance of a \textit{safe set} $\mathcal{C} \subset \R^{n}$, defined as the 0-superlevel set of a continuously differentiable function $h:\R^{n}\times\R^p\to\R$: 
\begin{equation}
    \mathcal{C} = \{ \mb{x} \in \R^{n} : h(\mb{x},\bs{\rho}) \geq 0 \}, \label{eq:safe_set}
\end{equation}
where the constant $\bs{\rho}\in\R^p$ is a set of parameters. We formally define safety as follows:
\begin{definition}[Forward Invariance and Safety \citep{ames2017control}] \label{def:CBF}
    Let $\bs{\rho}\in\R^p$ and let $\mathcal{C} \subset \R^{n}$ be defined as in \eqref{eq:safe_set}. The set $\mathcal{C} \subset \R^{n}$ is forward invariant if for every $\mb{x}_0 \in \mathcal{C}$ the solution $\mb{x}(t)$ to \eqref{eq:closed_loop_system} satisfies $\mb{x}(t) \in \mathcal{C}$ for all $t \geq 0 $. The system \eqref{eq:closed_loop_system} is safe with respect to $\mathcal{C}$ if $\mathcal{C}$ is forward invariant. 
\end{definition}

While it may possible to synthesize controllers that render a given set $\C$ safe in the presence of disturbances \citep{jankovic2018robust}, this may result in overly-conservative behavior. Instead, we consider how safety properties degrade with disturbances via the following definition:

\begin{definition}[Input-to-State Safety (ISSf) \citep{kolathaya2018input}]
\label{def:issf}
    % Given a set ${\mathcal{C} \subset \mathcal{Z}}$ that is the 0-superlevel set of a continuously differentiable function $h : \mathcal{Z} \to \R$,
    % and an open set $\mathcal{D}$, such that $\mathcal{C} \subset \mathcal{D} \subseteq \R^n $,
    Let $\bs{\rho}\in\R^p$ and let $\mathcal{C} \subset \R^{n}$ be defined as in \eqref{eq:safe_set}.
    The system \eqref{eq:closed_loop_system} is input-to-state safe with respect to $\mathcal{C}$ if there exists $\gamma \in \mathcal{K}$ such that for all $\delta\in\R_{\geq 0}$ and $\mb{d}:\R_{\geq 0}\to\R^m$ satisfying $\Vert\mb{d}\Vert_\infty\leq\delta$, the set $\mathcal{C}_{\delta}\subset\R^n$ defined as: 
    \begin{align}
       \mathcal{C}_{\delta} = \{\mb{x} \in \R^{n} : h(\mb{x}, \bs{\rho}) \geq - \gamma(\delta)\},
    \end{align}
    is forward invariant.
\end{definition}
This definition requires that in the absence of disturbances ($\delta = 0$), the original set $\C$ is safe. In the presence of disturbances, a neighborhood of $\C$ is safe, rather than $\C$ itself. Given this definition, ISSf Control Barrier Functions (ISSf-CBFs) can be used to design controllers that ensure \eqref{eq:closed_loop_system} is input-to-state safe with respect to $\mathcal{C}$ and which regulate the size of the set $\mathcal{C}_{\delta}$:
\begin{definition}[Input-to-State Safe Control Barrier Function (ISSf-CBF) \citep{alan2021safe}]
    Let $\bs{\rho}\in\R^p$ and let $\mathcal{C} \subset \R^{n}$ be defined as in \eqref{eq:safe_set}.
    % Let $\mathcal{C} \subset \mathcal{Z}$ be the 0-superlevel set of a continuously differentiable function $h: \mathcal{Z} \to \R$ with 0 a regular value. 
    The function $h$ is an Input-to-State Safe Control Barrier Function (ISSf-CBF) for~(\ref{eq:reduced_model}) on $\C$ if there exist $\alpha\in\K_\infty^e$ and $\sigma\in\R_{>0}$ such that for all $\mb{x} \in \R^{n}$: 
    \begin{equation} \label{eq:issf_cbf_constraint}
        \sup_{\mb{v} \in \R^{m}}
        \underbrace{\derp{h}{\mb{x}}(\mb{x},\bs{\rho})\mb{f}(\mb{x})}_{L_\mb{f}h(\mb{x},\bs{\rho})} + \underbrace{\derp{h}{\mb{x}}(\mb{x},\bs{\rho})\mb{g}(\mb{x})}_{L_\mb{g}h(\mb{x},\bs{\rho})}\mb{v} > -\alpha(h(\mb{x},\bs{\rho})) + \sigma\Vert L_\mb{g}h(\mb{x},\bs{\rho}) \Vert^2, 
    \end{equation}
\end{definition}
We have the following resulting relating ISSf-CBFs to Input-to-State Safety:
\begin{theorem}[\cite{alan2021safe}]\label{thm:CBF}
    Let $\bs{\rho}\in\R^p$ and let $\mathcal{C} \subset \R^{n}$ be defined as in \eqref{eq:safe_set}.
    % Given a set $\mathcal{C} \subset \mathcal{Z}$ defined as the 0-superlevel set of a continuously differentiable function $h: \mathcal{Z} \to \R$, 
    If $h$ is an ISSf-CBF for \eqref{eq:reduced_model}, then any locally Lipschitz continuous controller $\mb{k}: \R^{n} \to \R^{m}$ such that for all $\mb{x} \in \R^{n}$:
    \begin{equation} \label{eq:issf_constraint}
        L_\mb{f}h(\mb{x},\bs{\rho}) + L_\mb{g}h(\mb{x},\bs{\rho})\mb{k}(\mb{x}) \geq -\alpha(h(\mb{x},\bs{\rho})) + \sigma \Vert L_\mb{g}h(\mb{x},\bs{\rho}) \Vert^2,
    \end{equation}
   renders the system \eqref{eq:reduced_model} ISSf with respect to $\mathcal{C}$ with
    $\gamma(\delta) = -\alpha^{-1}(-\delta^2/4\sigma)$ with $\alpha^{-1}\in\K_\infty^e$. 
\end{theorem}

The parameter $\bs{\rho}\in\R^p$ often contains information about the system's environment that designates a given state as safe or unsafe, such as the location and size of obstacles. In highly unstructured environments the system may need to form an estimate of $\bs{\rho}$, denoted by $\widehat{\bs{\rho}}\in\R^p$ from measurements of the environment, such as image data. It is frequently the case that the process of converting complex measurements such as images into the low-dimensional representation $\widehat{\bs{\rho}}$ is imperfect, leading to an error between the estimator $\widehat{\bs{\rho}}$ and the true value of $\bs{\rho}$.

Not only does this error prevent one from evaluating whether a given state $\mb{x}\in\R^n$ is safe or unsafe, but it also prevents one from evaluating whether a given controller $\mb{k}$ satisfies the inequality in \eqref{eq:issf_constraint}.















% In practice, estimates of $\bs{\rho}$ are often determined via perception. We model perception by assuming the existence of Lipschitz continuous functions $\mb{q}:\R^n \times \R^p \to \R^\ell $, $\mb{r}: \R^\ell \to \R^p$, and $\widehat{\mb{r}}:\R^\ell \to \R^p$ where $\mb{q}$ is the perception module which maps $(\mb{x},\bs{\rho})$ to a high-dimensional representation such as an image, $\mb{r}$ is the state estimator which extracts state information from  $\mb{q}(\mb{x},\bs{\rho})$, and $\widehat{\mb{r}}$ which is an innacurate model of $\mb{r}$. Although we consider a deterministic case of measurement uncertainty, we note that stochastic CBFs have been considered in \citep{clark2019control}. In the case of error-less perception the obstacle state is recovered exactly as $\bs{\rho} = \mb{r}(\mb{q}(\mb{x}, \bs{\rho}))$. In the more realistic case of inaccurate estimation, we assume bounded errors such that 
\begin{equation}
    \widehat{\bs{\rho}} = \widehat{\mb{r}}(\mb{q}(\mb{x}, \bs{\rho})) \textrm{ and } \Vert \widehat{\mb{r}}(\mb{q}(\mb{x}, \bs{\rho})) - \bs{\rho}\Vert \leq \epsilon, \forall \mb{\bs{\rho}} \in \R^p \textrm{ and some } \epsilon \in [0, \infty).
\end{equation}
 

% Although this only models error in the obstacle parameters and not the robot state, we note that safety for collision avoidance depends on the relative position of the robot and the obstacle, thus error in the robot state can be modeled as error in the perceived obstacle parameters.

% Since the system can only access the perceived obstacle parameters $\widehat{\bs{\rho}}$, we must design a safe controller which accounts for this uncertainty. Considering $\bs{\rho}$ to be an extension of the state space, we extend Lemma \ref{lem:safety_reduced_model} following the method of \cite{dean2020guaranteeing} to account for this error. 







% Given a nominal (but not necessarily safe) locally Lipschitz continuous controller $\mb{k}_{\rm d}:\R^{n} \to \R^{m}$, the inequality in \eqref{eq:issf_constraint} may enforced as a constraint in a quadratic program-based safety filter to generate a safety-critical controller that guarantees ISSf: 
% \begin{align}
% \label{eqn:ISSf-CBF-QP}
% \tag{ISSf-CBF-QP}
% \mb{k}(\mb{x}) =  \,\,\underset{\mb{v} \in \R^{m}}{\argmin}  &  \quad \frac{1}{2} \Vert \mb{v} - \mb{k}_{\rm d}(\mb{x})\Vert^2  \\
% %\tag{CLF}
% \mathrm{s.t.} \quad & \quad L_\mb{f}h(\mb{x}) + L_\mb{g}h(\mb{x})\mb{v}
% \geq -\alpha(h(\mb{x}))  + \epsilon \Vert L_\mb{g}h(\mb{x}) \Vert^2. \nonumber
% \end{align}

% Intuitively, if an ISSf system has no disturbances ($\bs{\eta}(t) \equiv \mb{0}$), then $\mathcal{C} = \mathcal{C}_{\bs{\eta}}$ and the system is safe. For any disturbance $\Vert \bs{\eta} \Vert_\infty >0 $, a neighborhood $\mathcal{C}_{\bs{\eta}}$ of $\mathcal{C}$ is forward invariant ($\mathcal{C} \subset \mathcal{C}_{\bs{\eta}}$). 

% \subsection{Control Barrier Functions}
% Given $\mathcal{C}$ as the 0-superlevel set of $h$,  control barrier functions (CBFs) are tools which can be used to design controllers which ensure the safety of \eqref{eq:full_system}. 
% \begin{definition}[Control Barrier Function (CBF) \citep{ames2017control}]
%     Let $\mathcal{C} \subset \mathcal{Z}$ be the 0-superlevel set of a continuously differentiable function $h: \mathcal{Z} \to \R$ with 0 a regular value. The function $h$ is a control barrier function (CBF) if there exists an $\alpha \in \mathcal{K}$ such that for all $z \in \mathcal{Z}$: 
%     \begin{equation} \label{eq:cbf_constraint}
%         \sup_{u \in \R^{m}} \dot{h}(z,u) =  \frac{\partial h(z)}{\partial z} (F(z) + G(z) u) = L_fh(z) + L_gh(z)u \geq -\alpha(h(z)), 
%     \end{equation}
%     where $L_fh$ and $L_gh$ are Lie derivatives.
% \end{definition}
% Given a CBF $h$ for \eqref{eq:full_system}, we have the following result for the safety of the system: 
% \begin{theorem}[\cite{ames2017control}]\label{thm:CBF}
%     Given a set $\mathcal{C} \subset \mathcal{Z}$ defined as the 0-superlevel set of a continuously differentiable function $h: \mathcal{Z} \to \R$, if $h$ is a CBF for \eqref{eq:full_system}, then any Lipschitz continuous controller $k: \mathcal{Z} \to \R^{m}$, such that $u=k(z)$ satisfies \eqref{eq:cbf_constraint} for all $z \in \mathcal{C}$, renders the system safe with respect to the set $\mathcal{C}$. 
% \end{theorem}

% Given a nominal (but not necessarily safe) locally Lipschitz continuous controller $k_{\rm d}:\mathcal{Z} \to \R^{m}$, the CBF constraint \eqref{eq:cbf_constraint} can be used as a safety filter to generate the safety-critical CBF-QP controller: 
% \begin{align}
% \label{eqn:CBF-QP}
% \tag{CBF-QP}
% k(z) =  \,\,\underset{u \in \R^{m}}{\argmin}  &  \quad \frac{1}{2} \Vert u - k_{\rm d}(z)\Vert^2  \\
% %\tag{CLF}
% \mathrm{s.t.} \quad & \quad \dot{h}(z,u)
% \geq -\alpha(h(z)). \nonumber
% \end{align}


==> Sections/Maegans_PBL_text.tex <==

\section{Learning Framework}
Traditionally, user parameters such as $A,B,C,$ and $D$ require an expert human operator to make assumptions about an underlying utility function $U$ which may be difficult due to the indirect relationship between the parameters and the resulting trajectory of the system. Additionally, since $U$ is likely to balance desired performance with safety it admits no obvious mathematical description, several reward-based methods have developed explicit functions for $U$ \textcolor{blue}{CITE}. Our method shifts the responsibility of determining the safety-performance tradeoff from the engineer to the user. 

Alternatively, we propose the use of preference-based learning to rank the parameters from a set of three and also to label each set of parameters safe or unsafe. This uses the human's ability to identify ``ground-truth" safety even when unknown to the robot and also leaves the choice of the safety-performance balance to the user. 

\subsection{Learning Parameters}
We select the following parameters to learn, termed an action, $\act = [A,B,C,D] \in \R^4$. Each parameter is discretized and bounded, leading to a discrete search space given by the set $\actspace$.

The preference-based learning approach utilized here stems from the dueling bandit setting \citep{yue2012k} in which only pairwise comparison feedback is obtained from the system. Preference-based learning has recently been demonstrated in the context of robotic locomotion, where human preferences are collected and the robotic behavior is optimized to maximize an unknown objective function of the human. The main benefit of preference-based learning is that it searches complex parameter spaces without needing to explicitly define the underlying reward function. This is particularly useful in situations where the structure of the underlying reward function is unknown or not well understood. In these situations, poorly defined reward functions have been shown to result in “reward hacking” \citep{amodei2016concrete}, in which undesirable actions achieve high rewards. Alternatively, pairwise comparisons reliably capture the user's true intentions.


In our work, we specifically use the CoSpar algorithm \citep{tucker2020preference}, which iteratively selects actions to execute on the system, queries the human for pairwise preferences and suggestions, and updates its belief of the underlying utility function using Bayesian inference. The novelty of the CoSpar algorithm is that it operates in a 'mixed-initiative' setting by both providing believed optimal actions to the user (system-initiated), and asking the user for suggested optimal actions (user-initiated). 

In the following subsections, we will detail each of the three main steps of the learning approach: selecting new actions to sample, modeling human feedback, and approximating the underlying utility function.


\subsection{Selecting New Actions to Sample}
In each iteration, the algorithm selects one new action to sample in order to compare it with the previous action $(n = 1, b = 1)$. This method was first presented in \cite{tucker2020preference} as the 'buffer method'. In the first iteration a random action is sampled. In each subsequent iteration, a new action is sampled using Thompson sampling. Note that any sampling method designed for the bandit setting (in which the goal is to minimize cumulative regret) would also be acceptable, but the CoSpar algorithm specifically leverages Thompson sampling because it has been shown to have desirable behavior towards regret minimization \cite{chapelle2011empirical}. 

In general, the procedure of Thompson sampling in each iteration is the following. For each new action a sample is drawn from the posterior: $\r_{samp} \sim \P(\r, \data)$, and the action maximizing the drawn sample is selected to execute on the system: $\act_{samp} = \argmax \r_{samp}$

\subsection{Modeling Human Feedback}
After executing a new action on the system, the human operator is queried for two forms of subjective feedback: pairwise preferences and user suggestions. When using the buffer method, pairwise preferences are obtained by asking the user ``Do you prefer this action more or less than the last action?''. In the case where the user prefers action $\act_{1}$ to $\act_2$, this preference is denoted $\act_1 \succ \act_2$. Given the unknown utility function $r: \R^4 \to \R$, a single preference can be modeled using the likelihood function:
\begin{align*}
    \P(\act_1 \succ \act_2 \mid r(\act_1), r(\act_2)) = g\left( \frac{r(\act_1) - \r(\act_2)}{c_p} \right)
\end{align*}
where $g(\cdot): \R \to [0,1]$ is any monotonically-increasing link function, and $c_p > 0$ accounts for the expected noisiness of the provided preferences. In this work, we select $g(\cdot)$ to be the sigmoid function $g(\act) = 1/(1+\exp(-\act))$.

The likelihood function for a collection of $K$ preferences, defined as $\data_p$, can then be modeled as the product of each individual preference likelihood:
\begin{align*}
    \P(\data_p \mid r) = \prod_{k=1}^K \P(\act_{k1} \succ \act_{k2} \mid r(\act_{k1}), r(\act_{k2})),
\end{align*}
where $\act_{k1}$ and $\act_{k2}$ denote the preferred and non-preferred actions respectively for the $k^{\text{th}}$ pairwise preference.

User suggestions, formally termed coactive feedback \cite{shivaswamy2015coactive}, are incorporated into the learning framework as additional pairwise preferences in which the human suggests a `preferred' action to the currently executed action. The assumption is that the user \textit{would} prefer the suggested action if it was executed on the system. As with preferences. the likelihood function for a suggested action $\bar{\act}$ in comparison with an executed action $\act$ is modeled as:
\begin{align*}
    \P(\bar{\act} \succ \act \mid r(\bar{\act}), r(\act)) = g\left( \frac{r(\bar{\act}) - \r(\act)}{c_c} \right),
\end{align*}
where again $g(\cdot)$ is chosen to be the sigmoid function, and $c_c > 0$ quantifies noise in the user suggestions. Since suggestions are inherently prone to noise since the suggested action is not physically demonstrated on the system, we set $c_c > c_p$.

The likelihood function for a collection of $L$ suggestions is computed as the product of the individual likelihoods:
\begin{align*}
    \P(\data_c \mid r) = \prod_{l = 1}^{L} \P(\bar{\act_l} \succ \act_l \mid r(\bar{\act_l}), r(\act_l)),
\end{align*}
where $\bar{\act}_l$ and $\act_l$ are the suggested and executed action for the $l^{\text{th}}$ suggestion in the dataset. Assuming conditional independence, the combined likelihood function for all collected data $\data = \data_p \cup \data_c$ is then computed as $\P(\data \mid r) = \P(\data_p \mid r)\P(\data_c \mid r)$.

\subsection{Approximating the Underlying Utility Function}
The goal of the update step is to approximate the discrete set of utilities corresponding to the actions in $\actions$, denoted $\r \in \R^{|\actions|}$, as the maximum a posteriori (MAP) estimate $\hat{\r} = \argmax_{\r} \P(\r \mid \data)$. The posterior is approximated using the Laplace approximation as a Gaussian distribution $\P(\r \mid \data) \sim \mathcal{N}(\mu,\Sigma)$. Thus, the MAP estimate is approximated by $\hat{\r} \approx \mu$. 

\subsection{Safe Exploration with Preference-Based Learning}
\cite{sui2015safe} introduced the notion of \textit{safe exploration} in the context of sequential decision making, where a numerical reward signal was required to ensure that for all iterations $i$, some safety threshold condition is satisfied: $\r(\act) \geq h$ where $h \in \R$ is some problem-specific \textit{safety threshold}. Since the purpose of preference-based learning is to eliminate the need to utilize numerical rewards, we instead leverage the approach to safety introduced in \cite{li2021roial}.
\textcolor{blue}{TODO: Maegan}


==> Sections/NLPrelims.tex <==
In this section we formalize robust safety and discuss safe controller synthesis through the use of Control Barrier Functions (CBFs).
Consider the following nonlinear control-affine control system:
\begin{equation}
    \dot{\mb{x}} = \mb{f}(\mb{x}) + \mb{g}(\mb{x}) (\mb{v}+\mb{d}(t)),
    \label{eq:reduced_model}
\end{equation}
with state ${\mb{x} \in \R^{n}}$,
input ${\mb{v} \in \R^{m}}$, piecewise continuous disturbance signal ${\mb{d}(t):\R_{\geq 0} \to \R^{m}}$, and functions ${\mb{f}:\R^{n}\to\R^{n}}$ and ${\mb{g} : \R^{n}\to\R^{n \times m}}$ assumed to be locally Lipschitz continuous on their domains. Given a state-feedback controller $\mb{k}:\R^{n} \to \R^{m}$ that is locally Lipschitz continuous on its domain, setting the input $\mb{v} = \mb{k}(\mb{x})$ yields the closed-loop system:
\begin{equation}
    \dot{\mb{x}} = \mb{f}(\mb{x}) + \mb{g}(\mb{x}) (\mb{k}(\mb{x})+\mb{d}(t)).
    \label{eq:closed_loop_system}
\end{equation}
We assume that for any initial condition ${\mb{x}(0) = \mb{x}_0 \in \R^{n}}$ this system has a unique solution $\mb{x}(t)$ \citep{perko2013differential} that exists for all $t \in \R_{\geq 0}$. We denote $\Vert \cdot \Vert$ as the Euclidean norm and define $\Vert\mb{d}\Vert_{\infty} \triangleq \sup_{t \geq 0} \Vert\mb{d}\Vert$. We say that a continuous function ${\alpha : \R_{\geq 0} \to \R_{\geq 0}}$ is {\em class~$\mathcal{K}_\infty$} (${\alpha \in \mathcal{K}_\infty}$) if ${\alpha(0) = 0}$, $\alpha$ is strictly monotonically increasing, and $\lim_{r\to\infty}\alpha(r) = \infty$. We say that a continuous function $\alpha : \R \to \R$ is {\em class~$\mathcal{K}^{e}_\infty$} (${\alpha \in \mathcal{K}^e_{\infty}}$) if ${\alpha(0) = 0}$, $\alpha$ is strictly monotonically increasing, $\lim_{r\to\infty}\alpha(r) = \infty$, and $\lim_{r\to-\infty}\alpha(r) = -\infty$.



==> Sections/ObstacleUncertainty.tex <==
% In this section we modify the constraint \eqref{eq:desired_velocity_ISSf} and extend the result of Lemma \ref{lem:safety_reduced_model} to account for the effect of measurement uncertainty on safety, such as uncertainty in camera measurements for obstacle detection.

% % Previously, we considered the safe set $S = \{ z\in \mathcal{Z} : h(x) \geq 0 \} $. In practice, safe sets are often defined to ensure obstacle avoidance. To do so, the $h$ must also be a function of the parameters of the obstacle $\bs{\rho} \in \R^p$ which we assume to be constant. We can then extend the barrier functions to explicitly account for the obstacle parameters as $h_\textrm{obs}: \R^{k\times p} \to \R$, similarly the safe set becomes 
% % \begin{equation}
% % \mathcal{S}_\textrm{obs} = \{ z \in \mathcal{Z} : h_{\textrm{obs}}(x,\bs{\rho}) \geq 0 \}.
% % \end{equation}
% \textcolor{orange}{The mapping here should probably be from the trajectory x(t) \textit{signal} since we're using SLAM. What's the notation for that?}
% In practice, estimates of $\bs{\rho}$ are often determined via perception. We model perception by assuming the existence of Lipschitz continuous functions $\mb{q}:\R^n \times \R^p \to \R^\ell $, $\mb{r}: \R^\ell \to \R^p$, and $\widehat{\mb{r}}:\R^\ell \to \R^p$ where $\mb{q}$ is the perception module which maps $(\mb{x},\bs{\rho})$ to a high-dimensional representation such as an image, $\mb{r}$ is the state estimator which extracts state information from  $\mb{q}(\mb{x},\bs{\rho})$, and $\widehat{\mb{r}}$ which is an innacurate model of $\mb{r}$. Although we consider a deterministic case of measurement uncertainty, we note that stochastic CBFs have been considered in \citep{clark2019control}. In the case of error-less perception the obstacle state is recovered exactly as $\bs{\rho} = \mb{r}(\mb{q}(\mb{x}, \bs{\rho}))$. In the more realistic case of inaccurate estimation, we assume bounded errors such that 
% \begin{equation}
%     \widehat{\bs{\rho}} = \widehat{\mb{r}}(\mb{q}(\mb{x}, \bs{\rho})) \textrm{ and } \Vert \widehat{\mb{r}}(\mb{q}(\mb{x}, \bs{\rho})) - \bs{\rho}\Vert \leq \epsilon, \forall \mb{\bs{\rho}} \in \R^p \textrm{ and some } \epsilon \in [0, \infty).
% \end{equation}
 

% Although this only models error in the obstacle parameters and not the robot state, we note that safety for collision avoidance depends on the relative position of the robot and the obstacle, thus error in the robot state can be modeled as error in the perceived obstacle parameters.

% Since the system can only access the perceived obstacle parameters $\widehat{\bs{\rho}}$, we must design a safe controller which accounts for this uncertainty. Considering $\bs{\rho}$ to be an extension of the state space, we extend Lemma \ref{lem:safety_reduced_model} following the method of \cite{dean2020guaranteeing} to account for this error. 

\begin{definition}[\newcbf]
    Let $\mathcal{S}$ be as in \eqref{eq:safe_set_ro}.
    % Let $\mathcal{S} \subset \R^n\times\R^p$ be the 0-superlevel set of a continuously differentiable function ${h:\R^n \times \R^p \to \R}$ with 0 a regular value. 
    The function $h$ is a \newcbf for (\ref{eq:full_system}) with parameter function $\delta:\R^n \times \R^p \times \R^m  \to \R_{>0}$ if there exists $a>0$ such that for all $\bs{\rho} \in \R^p$ and all $\mb{x} \in \R^n$:
    %$(x, \widehat{x}_\textrm{obs}) \in \mathcal{S}$:
    \begin{align}
        \sup_{\mb{v}\in \R^l} L_\mb{f}h_R(\mb{x}, \widehat{\bs{\rho}}) + L_\mb{g}h_R(\mb{x},  \widehat{\bs{\rho}}) \mb{v} \geq  - a h_R(\mb{x},  \widehat{\bs{\rho}}) + \delta( \mb{x}, \widehat{\bs{\rho}}, \mb{v})   \label{eq:MRCBF-constraint}
    \end{align}
    % \begin{align}
    %     \sup_{v\in \R^k} L_fh(x, \widehat{x}_\textup{obs}) + L_gh(x, \widehat{x}_\textup{obs}) v  - \sigma \Vert L_gh \Vert^2 - \epsilon(\mathcal{L}_{L_fh} + \mathcal{L}_{\alpha h } + \mathcal{L}_{\sigma \Vert L_gh \Vert^2} + \mathcal{L}_{L_gh} \Vert  v \Vert ) \geq - \alpha h(x, \widehat{x}_\textup{obs}) \label{eq:MRCBF-constraint}
    % \end{align}
    %where $\epsilon\geq \Vert \bs{\rho} - \widehat{x}_\textrm{obs} \Vert  $.% and $\mathcal{L}$ represents the Lipschitz constant of the subscripted functions. 
\end{definition}
% As presented in the Appendix \ref{apdx:thm_proof}, satisfying this constraint guarantees that \eqref{eq:desired_velocity_ISSf} holds even if $\bs{\rho}$ is not known directly. 
By correctly choosing the function $\delta$, this allows us to consider measurement uncertainty in addition to the tracking error and disturbance of Lemma \ref{lem:safety_reduced_model}. This is summarized in the following theorem:

\begin{theorem} \label{thm:all_uncertainties}
Consider system (\ref{eq:full_system}), $\bs{\eta}$, $a$, and $b$ as in Lemma \ref{lem:safety_reduced_model}. If the velocity $\mb{v}$ satisfies \eqref{eq:MRCBF-constraint} with parameter function 
\begin{equation}
    \delta(\mb{x}, \widehat{\bs{\rho}}, \mb{v}) = b \Vert L_\mb{g}h_R(\mb{x}, \widehat{\bs{\rho}}) \Vert^2 + c + d  \Vert \mb{v} \Vert\label{eq:param_func}
\end{equation}
where $ c= \epsilon(\mathcal{L}_{L_\mb{f}h_R} + \mathcal{L}_{a h_R} + \mathcal{L}_{b \Vert L_\mb{g}h_R \Vert^2}) $, $d = \epsilon\mathcal{L}_{L_\mb{g}h_R} $, and $\mathcal{L}$ represents the Lipschitz constant of the subscripted functions, then $\mathcal{S}$ as defined in \eqref{eq:invariant_set} is ISSf for system \eqref{eq:full_system}.
\end{theorem}
\noindent A proof of this theorem can be found in Appendix \ref{apdx:thm_proof}. 

% We consider a Lipschitz continuous controller $v_{\rm nom}\triangleq\mu(z)$ where $\mu:\mathcal{Z}\to\R^l$ is designed to prioritize a goal without considering the safety tasks such as reaching to a point in 2D space without avoiding obstacles in environment.
To satisfy the conditions of Theorem \ref{thm:all_uncertainties}, we propose the following controller that operates as a safety filter similar to the \ref{eqn:ISSf-CBF-QP}:
\begin{align}\tag{\newcbf-OP}
\label{eq:new_controller}
\mb{k}(\mb{x}) = {\rm arg}\!\min_{\mb{v} \in \R^m } & \quad \Vert \mb{v} - \mb{v}_{\rm nom} \Vert^2  \\
   \textrm{s.t. } & L_\mb{f}h_R(\mb{x}, \widehat{\bs{\rho}}_i) + L_\mb{g}h_R(\mb{x},  \widehat{\bs{\rho}}_i) \mb{v} \geq  - a h_R(\mb{x},  \widehat{\bs{\rho}}_i) + \delta(\mb{x}, \widehat{\bs{\rho}}_i, \mb{v}), \quad \forall i \in \{1, \dots, I\}  \nonumber
\end{align}
where $\delta$ is as defined in \eqref{eq:param_func} and $\widehat{\bs{\rho}}_i$ indicates the measured parameters of obstacle $i$ with $I \in \mathbb{N}_{\geq 0}$ being the total number of obstacles. Enforcing this constraint for $I>1$ results in taking the intersection of the safe sets as outlined in \citep{glotfelter2018boolean}. 
% This controller utilizes the simple reduced-order system \eqref{eq:reduced_model} and ensures that controller output $\mb{v}_{\rm \mb{d}}$ satisfies the condition \eqref{eq:MRCBF-constraint} with the constraint.
The safety filter is a Second-Order Cone Program (SOCP) \citep{boyd2004convex} for which an array of solvers exist including ECOS \citep{domahidi2013ecos}. CBF-based SOCP safety filters have shown success on embedded systems in \cite{cosner2021measurement}. Infeasibilities of this optimization problem can be overcome through the use of a slack variable, the impact of which on safety can be understood through the lense of projection-to-state safety \cite{taylor2020control}.
% which has been shown to be a computationally tractable for embedded systems as a similar controller was demonstrated in \citep{cosner2021measurement}.






Theorem \ref{thm:all_uncertainties} accounts for the disturbance $\mb{d}$, the measurement uncertainty in  $\widehat{\bs{\rho}}$, and the reduced-order structure of (\ref{eq:full_system}) and states that any input that satisfies the \eqref{eq:MRCBF-constraint} will render $\mathcal{S}_e $ ISSf.
However, the variables $a, b, c, d >0$ are all either user defined parameters or bounds which may be difficult to ascertain. Additionally, although values of these parameters exist to guarantee safety (assuming feasibility of the constraint), such values may be highly conservative and lead to undesirable behavior. The parametric nature of the \newcbf thus provides a nice structure for which \newpbl can be deployed to determine the user-preferred balance of performance with safety. 

% However, in general the upper bound on $a$, the lower bound on $b$, and the measurement error robustification terms $c$ and $d$ are all unknown or user-defined parameters. 


% Additionally, achieving guaranteed safety using the true values of these parameters might be unnecessarily conservative. Therefore in order to achieve a user-desired balance between performance and robust safety we use preference-based learning to determine user-preferred values of $a,b,c,$ and $d$.

==> Sections/RO_models.tex <==
% In this section we consider a simplified reduced-order model of \eqref{eq:full_system}, analyze the effect of this additional structure and measurement uncertainty on safety, and propose a controller which guarantees the input-to-state safety of the full system \eqref{eq:full_system}.

In this section we define the safety-critical control problem for complex systems through the lens of ISSf-CBFs.
We discuss how robustness to disturbances and measurement error may be incorporated into controller synthesis, to ultimately achieve safety in practice.
To simplify robust safety-critical control design, we rely on reduced-order models.

While real-life engineering systems may have complex dynamics with high-dimensional state space, often not all states affect safety.
Therefore, we consider systems where the states can be separated into two groups:
states ${\mb{x} \in \R^{n}}$ that directly affect safety and the rest of the states ${\bs{\xi} \in \R^{k}}$.
% We assume that: (i) the dynamics of $\mb{x}$ can be captured by a reduced-order model; (ii) the dynamics of $\bs{\xi}$ are controlled by a low-level control input $\mb{u} \subseteq \R^l$.
Accordingly, we consider the following nonlinear control-affine cascaded system:
\begin{align}
\begin{split}
    \dot{\mb{x}} &= \mb{f}(\mb{x})+\mb{g}(\mb{x})\bs{\kappa}(\bs{\xi}), \\
 \dot{\bs{\xi}} &= \mb{f}_{\bs{\xi}}(\mb{x},\bs{\xi}) + \mb{g}_{\bs{\xi}}(\mb{x},\bs{\xi})\mb{u},
 \end{split}
 \label{eq:full_system}
\end{align}
with control input $\mb{u} \in \R^l$ and functions
${\mb{f}:\R^n \to \R^n}$,
${\mb{g}: \R^n \to \R^{n \times m}}$,
$\bs{\kappa}: \R^k \to \R^m$, $\mb{f}_{\bs{\xi}}:\R^n \times \R^k \to \R^k$, and
$\mb{g}_{\bs{\xi}}:\R^n \times \R^k \to \R^{n \times l}$ assumed to be locally Lipschitz continuous on their domains.
% {\color{blue}TM: I feel here the overall right-hand side for $\dot{\mb{x}}$ is given by the problem, $\mb{f}$ and $\mb{g}$ are something that we choose when choosing a reduced-order model, and this choice affects the expression of $\bs{\kappa}$ (and it must be a valid choice...).}
These dynamics may represent systems described by the Euler-Lagrange equations, such as robotic systems, where $\mb{x}$ reflect position coordinates affecting safety, $\bs{\xi}$ involves velocity and not safety-critical position coordinates, and the input $\mb{u}$ reflects forces and torques applied to the system. 
% \begin{align}
%     \dot{\mb{z}} \lmat \dot{\mb{x}} \\ \dot{\mb{y}} \rmat & = \mb{F}(\mb{z}) + \mb{G}(\mb{z})(\mb{u}) + \mb{d}) 
% \end{align}

Motivated by \cite{molnar2021model}, this cascaded model is taken for two reasons.
The first reason is that the dynamics of the state $\bs{\xi}$ may often be very complicated, such as in the case of legged locomotion \AT{CITE}.
Thus it is often the case that the control of these dynamics is treated as a separate subsystem. 
The second reason is that many safety requirements (such as collision-avoidance) are specified as constraints on position, state $\mb{x}$, rather than on both states $\mb{x}$ and $\bs{\xi}$. 
We consider that the cascaded system is associated with the safe set:
\begin{equation}
    \mathcal{S} = \{ (\mb{x},\bs{\xi}) \in \R^n \times \R^k : h_R(\mb{x}, \bs{\rho}) \geq 0 \},    \label{eq:safe_set_ro}
\end{equation}
defined by a continuously differentiable function ${h_R : \R^n \times \R^p  \to \R}$ and some constant parameters $\bs{\rho} \in \R^p$ associated with the problem ($\dot{\bs{\rho}}=0$).

==> Sections/RO_safety.tex <==

% For safety, we consider the case where safety is affected only by the reduced-order state $\mb{x}$ and some parameters $\bs{\rho}\in\R^p$ which we assume to be constant (i.e. $\frac{\textrm{d}\bs{\rho}}{\textrm{d} t}=0$).
% This safe set is given by:
% \begin{equation}
%     \mathcal{S} = \{ \mb{z} \in \mathcal{Z} : h_R(\mb{x}, \bs{\rho}) \geq 0 \},
%     \label{eq:safe_set_ro}
% \end{equation}
% with a continuously differentiable function ${h_R : \mathcal{X}\times \R^p  \to \R}$.
% For example, in 2D obstacle avoidance with the Cassie robot,  $\bs{\rho}$ represents the size and location of obstacles, $z$ is the full state of Cassie (with ${n=...}$ dimensions), while safety is primarily influenced by its planar position $x$ (with ${k=2}$ dimensions).


To facilitate robust safety-critical control, we consider~(\ref{eq:reduced_model}) as a reduced-order model for~(\ref{eq:full_system}), and we achieve safety by a two-layer control architecture.
First, we design a safe velocity reference $\mb{v}=\mb{k}(\mb{x})$ based on the reduced-order model~(\ref{eq:reduced_model}) using the ISSf-CBF construction.
Second, we apply a low-level velocity tracking controller
$\mb{u} = \Theta(\mb{x},\bs{\xi}), \Theta: \R^n \times \R^k \to \R^l$
designed for the full system~(\ref{eq:full_system}) such that $\bs{\kappa}(\bs{\xi})$ tracks the reference $\mb{v}$.
The two layers are linked by the tracking error $\mb{d}$:
\begin{equation}
    \mb{d} \triangleq \kappa(\bs{\xi}) - \mb{v},
    \label{eq:tracking_error}
\end{equation}
which act as disturbance on the reduced-order model~(\ref{eq:reduced_model}) and which the low-level controller of the full system~(\ref{eq:full_system}) intends to eliminate.
We assume the existence of a low-level velocity tracking controller $\mb{u}$ that ensures bounded tracking of $\mb{v}$. 
% there exists an ISS tracking controller which exponentially reduces $V(\eta)$ to a neighborhood of zero. 

\begin{figure}
    \centering
    \includegraphics[width=0.25\linewidth]{Figures/Issf.png}
    \includegraphics[width=0.3\linewidth]{Figures/unitreeA1.png}
    \includegraphics[width=0.4\linewidth]{Figures/velocity_tracking.png}
    % \includegraphics[width=3cm,height=5cm]{Figures/20211029_184621.jpg}
    \caption{(\textbf{Left})  Visualization of the ISSf property and the effect of disturbances on the safe set. (\textbf{Center}) The Unitree A1 robot used in simulation and experiments. (\textbf{Right}) Velocity tracking of the Unitree A1 robot. This shows the forward and angular velocities throughout an experiment and demonstrates the bounded tracking assumed in Assumption \ref{assp:ISS-tracking}.}
    \label{fig:ISS_exp_proof}
\end{figure}

\begin{assumption} \label{assp:ISS-tracking}
The low-level tracking controller ${\mb{u} = \Theta(\mb{\mb{x},\bs{\xi}})}$, ${\Theta : \R^n \times \R^k \to \R^l}$, ensures that $\Vert \mb{d} \Vert_\infty \leq \delta $ for some $\delta\in\R_{\geq 0}$ for the full system \eqref{eq:full_system}. 
% allows input-to-state stable tracking, i.e. there exists $ M, \beta \in \R_{>0}$ and $\mu \in \mathcal{K}$ such that \eqref{eq:ISS} holds. 
% i.e., there exists a positive definite function ${V : \R^l \to \R_{\geq 0}}$, constants ${k_{1}, k_{2}, k_{3} \in \R_{>0}}$ and $\iota \in \mathcal{K}$ such that:
% \begin{align}
%     \begin{split}
%         k_{1} \| \eta \|^2&  \leq V(\eta) \leq k_{2} \| \eta \|^2, \\
%         \dot{V}(z,\Theta(z)) &  \leq -  k_{3} \| \eta \|^2 + \iota (\|d\|_{\infty}),
%     \end{split}
%     \label{eq:tracking_controller_ISS}
% \end{align}
% where ${\eta = \Phi(z)}$ and ${\dot{V}(z,\Theta(z)) = \frac{\partial V(\Phi(z))}{\partial z} (F(z) + G(z) (\Theta(z)+d))}$.
\end{assumption}

% \begin{assumption} \label{assp:ISS-tracking}
% The tracking controller ${u = \Theta(z)}$, ${\Theta : \mathcal{Z} \to \mathcal{U}}$ allows input-to-state stable tracking, i.e., there exists a positive definite function ${V : \R^l \to \R_{\geq 0}}$, constants ${k_{1}, k_{2}, k_{3} \in \R_{>0}}$ and $\iota \in \mathcal{K}$ such that:
% \begin{align}
%     \begin{split}
%         k_{1} \| \eta \|^2&  \leq V(\eta) \leq k_{2} \| \eta \|^2, \\
%         \dot{V}(z,\Theta(z)) &  \leq -  k_{3} \| \eta \|^2 + \iota (\|d\|_{\infty}),
%     \end{split}
%     \label{eq:tracking_controller_ISS}
% \end{align}
% where ${\eta = \Phi(z)}$ and ${\dot{V}(z,\Theta(z)) = \frac{\partial V(\Phi(z))}{\partial z} (F(z) + G(z) (\Theta(z)+d))}$.
% \end{assumption}

% For Cassie, we rely on the success of \citep{xiong20213d} that tracks desired longitudinal and lateral velocities given by $v_{\rm d}$ and show in Figure \ref{fig:ISS_exp_proof} experimental results demonstrating the ISS tracking capability of this controller. 

% The rest of the states, $\mb{y}$, do not directly affect point-wise safety. 
% For example, in the case of obstacle avoidance with the quadruped, safety may be encoded as simply the planar position of the robot without direct dependence on the joint positions. %The planar velocity $v$ of Cassie, however, does play an important role in the safety through time, and it is part of $y$.

% Since $L_\mb{G}h_R(\mb{z})\equiv0$ for system \eqref{eq:reduced_model} with $h_R$ as in \eqref{eq:safe_set}, we rely on the bounded tracking of Assumption \ref{assp:ISS-tracking} and treat such error $\Vert \eta \Vert >0$ as a matched disturbance. 
% we consider the extended function $h_e:\mathcal{Z}\times\R^p\to\R$ and associated safe set $\mathcal{S}_e\subseteq \subset \mathcal{S } \subset \mathcal{X}$ from \cite{molnar2021model}:
% \begin{align}
%     h_e(\mb{z}, \bs{\rho}) \triangleq - \frac{1}{4ab}\mu(\Vert \mb{d}\Vert_\infty ) +  \alpha_e h_R(\mb{x}, \bs{\rho}), % \label{eq:hV}
%     &&     \mathcal{S}_e \triangleq \{ \mb{z} \in \mathcal{Z} : h_e(\mb{z}, \bs{\rho}) \geq 0  \},    \label{eq:hV_and_SV}
% \end{align}
% where $V$ as in Assumption \ref{assp:ISS-tracking} and $\alpha_e > 0$.  \textcolor{orange}{How does this change with just the bound? }
% Based on the Definition~\ref{def:issf} we seek to get a safety certificate for a larger set in the presence of the disturbance $\Vert \mb{d} \Vert_\infty >0$. 
At the reduced-order model level, we enforce that the set $\mathcal{S}$ is ISSf with respect to the bounded and matched disturbance $\mb{d}$.
%given ISS tracking of the reduced-order input
The desired velocity $\mb{v}$ is designed so that it satisfies the ISSf-CBF constraint for the reduced-order dynamics:
\begin{equation}
    L_\mb{f}h_R(\mb{x},\bs{\rho}) + L_\mb{g}h_R(\mb{x},\bs{\rho}) \mb{v} \geq - a h_R(\mb{x}, \bs{\rho}) + b \Vert L_\mb{g}h_R(\mb{x},\bs{\rho}) \Vert^2 .
    % \frac{\partial h(x, \bs{\rho})}{\partial x} (f(x) + g(x) v_{\rm d}) \geq - \alpha h(x, \bs{\rho}) + \sigma \Vert L_gh(x,\bs{\rho}) \Vert^2 ,
    \label{eq:desired_velocity_ISSf}
\end{equation}
% where ${a, b \in \R_{>0}}$ are user-defined parameters. 
% We note that \eqref{eq:desired_velocity_ISSf} involves the function $h_R$, and the function $V$ is not required in the condition. Based on the existence of a function $V$ that satisfies Assumption \ref{assp:ISS-tracking} with a controller $\Theta(\mb{z})$ we make the following claim on the system \eqref{eq:full_system}.
Based on Assumption \ref{assp:ISS-tracking} we make the following claim on the safety of the full system \eqref{eq:full_system}. 

%We note that this is a linear constraint on $v_{\rm d}$, so \eqref{eq:desired_velocity_ISSf} can be incorporated as a constraint of an optimization-based controller as done with the \eqref{eqn:CBF-QP}.
% This gives a desired velocity $v_{\rm d}$ that depends on the reduced state $x$: ${v_{\rm d} = \Psi(x)}$, ${\Psi: \mathcal{X} \to \mathcal{V}}$.
%Given Assumption \ref{assp:ISS-tracking} and constraint \eqref{eq:desired_velocity_ISSf} we make the following claim on the system \eqref{eq:full_system}.

\begin{lemma} \label{lem:safety_reduced_model}
\textit{
Consider system~(\ref{eq:full_system}), velocity $\mb{v}$ satisfying~(\ref{eq:desired_velocity_ISSf}), tracking error $\mb{d}$ given by~(\ref{eq:tracking_error}), and a tracking controller $\mb{u}=\Theta(\mb{x},\bs{\xi})$ satisfying Assumption \ref{assp:ISS-tracking}.
%for a positive definite function $V$ as given in Assumption \ref{assp:ISS-tracking}.
%velocity tracking controller satisfying~(\ref{eq:tracking_controller_ISS}).
% $\mathcal{S}$ is ISSf and 
% the following set is forward invariant 
Then, $\mathcal{S}$ as defined in \eqref{eq:safe_set_ro} is ISSf, associated with the following forward invariant set:
% under~(\ref{eq:full_system}) 
% for all ${\alpha_{\rm e} > 0}$ with 
\begin{equation}
    \mathcal{S}_{\mb{d}} = \left\{ (\mb{x},\bs{\xi}) \in \R^n \times \R^k : h_R(\mb{x}, \bs{\rho}) \geq  - \frac{1}{4ab}\delta^2 \right\}.
    \label{eq:invariant_set}
\end{equation}
% for $b \geq \frac{\alpha_{\rm e}}{4(k_{3} - k_{2}a)}$ and ${0<a<k_{3}/k_{2}}$.
} 
% \textcolor{orange}{this is now just the standard ISSf-CBF theorem I think.}
\end{lemma}
Lemma \ref{lem:safety_reduced_model} directly follows from Theorem \ref{thm:CBF}, and its proof can be found in Appendix \ref{apdx:lemma_proof}.

% \begin{remark}
% Lemma \ref{lem:safety_reduced_model} implies that the set $\mathcal{S}_e$ is safe for ${\Vert \mb{d} \Vert_{\infty} = 0}$. Thus, for any initial conditions satisfying ${\mb{z}_{0} \in \mathcal{S}_{e}}$ we have ${\mb{z}(t) \in \mathcal{S}_{e}} \subseteq \mathcal{S}$ for all ${t \geq 0}$.
% %Lemma \ref{lem:safety_reduced_model} implies the following.
% %For zero disturbance (${\| d \|_{\infty} = 0}$) we have ${\mathcal{S}_{V} \subseteq S}$ since ${V(\eta) \geq 0}$.
% %Thus, for initial conditions satisfying ${z_{0} \in \mathcal{S}_{V}}$ we get ${z(t) \in \mathcal{S}_{V} \subset S}$, ${\forall t \geq 0}$, i.e., the system stays safe.
% Furthermore, even with the presence of disturbance (${\Vert \mb{d} \Vert_{\infty} > 0}$) the forward invariant set $\mathcal{S}_{e,\mb{d}}$ can be made arbitrarily close to $\mathcal{S}$ for a large $\alpha_{\rm e}$. 
% As ${\alpha_{\rm e} \to \infty}$, the expression of $h_{e}(\mb{z},\bs{\rho})$ in~(\ref{eq:hV_and_SV}) approaches $h_R(\mb{x},\bs{\rho})$, and the definition~(\ref{eq:invariant_set}) of $S_{e,\mb{d}}$ recovers the set $\mathcal{S}$ given as in~(\ref{eq:safe_set}).
% However, since a large $\alpha_{\rm e}$ proportionally yields a large lower bound on $b$, approaching the ideal safe behaviour results more strict condition for the tracking error $\eta$ to satisfy as the modification in~(\ref{eq:desired_velocity_ISSf}) becomes more prominent.
% %That is, by tuning $\sigma$ the deviation between $\mathcal{S}_{V}$ and $S$ can be reduced arbitrarily and we can get arbitrarily close to the ideal safe behavior despite disturbances.
% %This motivates tuning parameter $\sigma$ by learning.
% \end{remark}


==> Sections/old/ISSf.tex <==
We formalize the notion of safety as the forward invariance of a \textit{safe set} $\mathcal{C} \subset \mathcal{Z}$. The system is considered safe as long as $\mb{z}(t)$ remains in $\mathcal{C}$. In particular, we consider safe sets defined as the 0-superlevel sets of continuously differentiable functions $h : \mathcal{Z} \to \R$: 
\begin{equation}
    \mathcal{C} \triangleq \{ \mb{z} \in \mathcal{Z} : h(\mb{z}) \geq 0 \}, \quad
    \partial \mathcal{C} \triangleq \{ \mb{z} \in \mathcal{Z} : h(\mb{z}) = 0 \}, \quad
    \textrm{Int}( \mathcal{C}) \triangleq \{ \mb{z} \in \mathcal{Z} : h(\mb{z}) > 0 \} . \label{eq:safe_set}
\end{equation}
We can now formally define safety and forward invariance using these constructions.
\begin{definition}[Forward Invariance and Safety \citep{ames2017control}] \label{def:CBF}
    A set $\mathcal{C} \subset \mathcal{Z}$ is forward invariant if for every $\mb{z}_0 \in \mathcal{C}$ the solution $\mb{z}(t)$ to \eqref{eq:full_system} satisfies $\mb{z}(t) \in \mathcal{C}$ for all $t \geq 0 $. The system \eqref{eq:full_system} is safe with respect to $\mathcal{C}$ if $\mathcal{C}$ is forward invariant. 
\end{definition}

% The effects of disturbances on safety can be framed 
Considering the effect of disturbances on safety, we define input-to-state safety. 

\begin{definition}[Input-to-State Safety (ISSf) \citep{kolathaya2018input}]
\label{def:issf}
    % Given a set ${\mathcal{C} \subset \mathcal{Z}}$ that is the 0-superlevel set of a continuously differentiable function $h : \mathcal{Z} \to \R$,
    % and an open set $\mathcal{D}$, such that $\mathcal{C} \subset \mathcal{D} \subseteq \R^n $,
    Let $\mathcal{C} \subset \mathcal{Z}$ be defined as in \eqref{eq:safe_set}
    the set $\mathcal{C}$ is input-to-state safe, if there exists $\gamma \in \mathcal{K}$ such that the set $\mathcal{C}_d$ defined as: 
    \begin{align}
        \mathcal{C}_\mb{d} \triangleq \{ \mb{z} \in \mathcal{Z} : h(\mb{z}) \geq - \gamma(\Vert \mb{d} \Vert_\infty)\} 
    \end{align}
    is forward invariant. \textcolor{orange}{This was lifted out of the cited text, but it seems like the closed loop system is missing in this def.}
\end{definition}
Intuitively, if $\mathcal{C}$ is ISSf and the system has no disturbances ($\mb{d} \equiv \mb{0}$), then $\mathcal{C} = \mathcal{C}_\mb{d}$ and set $\mathcal{C}$ is safe. For any disturbance $\Vert \mb{d} \Vert_\infty >0 $, a neighborhood $\mathcal{C}_\mb{d}$ of $\mathcal{C}$ is forward invariant ($\mathcal{C} \subset \mathcal{C}_\mb{d}$). 

% \subsection{Control Barrier Functions}
% Given $\mathcal{C}$ as the 0-superlevel set of $h$,  control barrier functions (CBFs) are tools which can be used to design controllers which ensure the safety of \eqref{eq:full_system}. 
% \begin{definition}[Control Barrier Function (CBF) \citep{ames2017control}]
%     Let $\mathcal{C} \subset \mathcal{Z}$ be the 0-superlevel set of a continuously differentiable function $h: \mathcal{Z} \to \R$ with 0 a regular value. The function $h$ is a control barrier function (CBF) if there exists an $\alpha \in \mathcal{K}$ such that for all $z \in \mathcal{Z}$: 
%     \begin{equation} \label{eq:cbf_constraint}
%         \sup_{u \in \mathcal{U}} \dot{h}(z,u) =  \frac{\partial h(z)}{\partial z} (F(z) + G(z) u) = L_fh(z) + L_gh(z)u \geq -\alpha(h(z)), 
%     \end{equation}
%     where $L_fh$ and $L_gh$ are Lie derivatives.
% \end{definition}
% Given a CBF $h$ for \eqref{eq:full_system}, we have the following result for the safety of the system: 
% \begin{theorem}[\cite{ames2017control}]\label{thm:CBF}
%     Given a set $\mathcal{C} \subset \mathcal{Z}$ defined as the 0-superlevel set of a continuously differentiable function $h: \mathcal{Z} \to \R$, if $h$ is a CBF for \eqref{eq:full_system}, then any Lipschitz continuous controller $k: \mathcal{Z} \to \mathcal{U}$, such that $u=k(z)$ satisfies \eqref{eq:cbf_constraint} for all $z \in \mathcal{C}$, renders the system safe with respect to the set $\mathcal{C}$. 
% \end{theorem}

% Given a nominal (but not necessarily safe) locally Lipschitz continuous controller $k_{\rm d}:\mathcal{Z} \to \mathcal{U}$, the CBF constraint \eqref{eq:cbf_constraint} can be used as a safety filter to generate the safety-critical CBF-QP controller: 
% \begin{align}
% \label{eqn:CBF-QP}
% \tag{CBF-QP}
% k(z) =  \,\,\underset{u \in \mathcal{U}}{\argmin}  &  \quad \frac{1}{2} \Vert u - k_{\rm d}(z)\Vert^2  \\
% %\tag{CLF}
% \mathrm{s.t.} \quad & \quad \dot{h}(z,u)
% \geq -\alpha(h(z)). \nonumber
% \end{align}

Given this definition, ISSf control barrier functions (ISSf-CBFs) are tools which can be used to design controllers that render \eqref{eq:full_system} safe with respect to $\mathcal{C}_\mb{d}$ and which regulate the size of the expansion $\mathcal{C}\subseteq \mathcal{C}_\mb{d}$.
\begin{definition}[Input-to-State Safe Control Barrier Function (ISSf-CBF) \citep{alan2021safe}]
    Let $\mathcal{C} \subset \mathcal{Z}$ be defined as in \eqref{eq:safe_set}.
    % Let $\mathcal{C} \subset \mathcal{Z}$ be the 0-superlevel set of a continuously differentiable function $h: \mathcal{Z} \to \R$ with 0 a regular value. 
    The function $h$ is an input-to-state safe control barrier function (ISSf-CBF) if there exist $a,b>0$ such that for all $\mb{z} \in \mathcal{Z}$: 
    \begin{equation} \label{eq:issf_cbf_constraint}
        \sup_{\mb{u} \in \mathcal{U}} \dot{h}(\mb{z},\mb{u})
        % =  \frac{\partial h(z)}{\partial z} (F(z) + G(z) u)
        = L_\mb{F}h(\mb{z}) + L_\mb{G}h(\mb{z})\mb{u} \geq -a h(\mb{z}) + b \Vert L_\mb{G}h(\mb{z}) \Vert^2, 
    \end{equation}
    where $L_\mb{F}h(\mb{z}) = \frac{\partial h(\mb{z})}{\partial z} \mb{F}(z)$ and $L_\mb{G}h(\mb{z}) = \frac{\partial h(\mb{z})}{\partial \mb{z}} \mb{G}(\mb{z})$ are Lie derivatives. \textcolor{orange}{Where's the set-shrinking part of this theorem using b? }
\end{definition}
Given an ISSf-CBF $h$ for \eqref{eq:full_system}, we have the following result for the input-to-state safety of the system.
\begin{theorem}[\cite{alan2021safe}]\label{thm:CBF}
    Let $\mathcal{C} \subset \mathcal{Z}$ be defined as in \eqref{eq:safe_set}.
    % Given a set $\mathcal{C} \subset \mathcal{Z}$ defined as the 0-superlevel set of a continuously differentiable function $h: \mathcal{Z} \to \R$, 
    If $h$ is an ISSf-CBF for \eqref{eq:full_system}, then any Lipschitz continuous controller $\mb{k}: \mathcal{Z} \to \mathcal{U}$, such that $\mb{u}=\mb{k}(\mb{z})$ satisfies \eqref{eq:issf_cbf_constraint} for all $\mb{z} \in \mathcal{Z}$, renders the system input-to-state safe with respect to the set $\mathcal{C}$. 
\end{theorem}

Given a nominal (but not necessarily safe) locally Lipschitz continuous controller $\mb{k}_{\mb{d}}:\mathcal{Z} \to \mathcal{U}$, the ISSf-CBF constraint \eqref{eq:issf_cbf_constraint} can be used as the constraint in a quadratic program-based safety filter to generate the safety-critical controller: 
\begin{align}
\label{eqn:ISSf-CBF-QP}
\tag{ISSf-CBF-QP}
\mb{k}(\mb{z}) =  \,\,\underset{\mb{u} \in \mathcal{U}}{\argmin}  &  \quad \frac{1}{2} \Vert \mb{u} - \mb{k}_{\mb{d}}(\mb{z})\Vert^2  \\
%\tag{CLF}
\mathrm{s.t.} \quad & \quad L_\mb{F}h(\mb{z}) + L_\mb{G}h(\mb{z})\mb{u}
\geq -a h(\mb{z})  + b \Vert L_\mb{G}h(\mb{z}) \Vert^2. \nonumber
\end{align}


==> Sections/old/NLPrelims.tex <==

% \begin{align}
%     \dot{\mb{x}} &= \mb{f}(\mb{x})+\mb{g}(\mb{x})\bs{\xi} \\ \dot{\bs{\xi}} &= \mb{f}_{\bs{\xi}}(\mb{x},\bs{\xi}) + \mb{g}_{\bs{\xi}}(\mb{x},\bs{\xi})\mb{u}
% \end{align}

% There exists $\mb{k}:\R^{n?}\to\R^m$ such that:
% \begin{equation}
%     \Vert \bs{\xi}-\bs{\xi}_d(t)\Vert \leq \epsilon
% \end{equation}


In this section we formalize robust safety and discuss safe controller synthesis through the use of control barrier functions (CBFs). For this work we consider the full-order dynamical system with
state ${\mathbf{z} \in \mathcal{Z} \subseteq \R^{n}}$,
input ${\mathbf{u} \in \mathcal{U} \subseteq \R^{m}}$ and
bounded disturbance ${\mathbf{d} \in \mathcal{D} \subseteq \R^{m}}$:
\begin{equation}
    \dot{\mathbf{z}} = \mb{F}(\mathbf{z}) + \mb{G}(\mathbf{z}) (\mb{u}+\mb{d}),
    \label{eq:full_system}
\end{equation}
where ${\mb{F} : \mathcal{Z} \to \R^{n}}$ and ${\mb{G} : \mathcal{Z} \to \R^{n \times m}}$ are Lipschitz continuous. Given the initial condition ${\mb{z}(0) = \mb{z}_0 \in \mathcal{Z}}$ and a Lipschitz continuous state-feedback controller $\mb{k}:\mathcal{Z} \to \mathcal{U}$, $\mb{u} = \mb{k}(\mb{z}) $, the system has a unique solution $\mb{z}(t)$ \citep{perko2013differential} which we assume exists for all $t \geq 0 $. 

Throughout the rest of this paper we use the notation that $\Vert \cdot \Vert$ denotes the Euclidean norm and $\Vert \cdot \Vert_\infty$ the maximum norm.
We say that a continuous function ${\alpha : [0,a) \to \R_{\geq 0}}$ with ${a>0}$ is {\em class $\mathcal{K}$} (${\alpha \in \mathcal{K}}$) and a continuous function ${\alpha : (-b,a) \to \R_{\geq 0}}$ with ${a,b>0}$ is {\em extended class $\mathcal{K}$} (${\alpha \in \mathcal{K}_{\rm e}}$) if $\alpha$ is strictly monotonically increasing and ${\alpha(0) = 0}$.


==> Sections/proposed_paradigm.tex <==
% Utilizing the notions of MR-CBFs

% \begin{definition}[Tunable Robust Control Barrier Function]
% The function $h$ is a \AT{Tunable Robust Control Barrier Function (TR-CBF)} for \eqref{eq:reduced_model_dist} on $\C$ with parameters $a,b,\sigma\in\R_{\geq 0}$ if there exist $\alpha\in\K_{\infty}^e$ such that for all $\widehat{\bs{\rho}}\in\R^p$ and $\mb{x}\in\R^n$:  
% \begin{equation}
%     \sup_{\mb{v}\in\R^m} L_{\mb{f}}h(\mb{x},\widehat{\bs{\rho}}) + L_{\mb{g}}h(\mb{x},\widehat{\bs{\rho}})\mb{v} -a -b\Vert\mb{v}\Vert - \sigma\Vert L_{\mb{g}}h(\mb{x},\widehat{\bs{\rho}})\Vert^2 > -\alpha(h(\mb{x},\widehat{\bs{\rho}}))
% \end{equation}
% \end{definition}









% To synthesize safe controllers for system \eqref{eq:full_system} we can combine the robustness properties presented in Theorems \ref{thm:mrcbf} and \ref{thm:issf-cbf} in a parametric format amenable to \newpbl. 

% In particular we propose \newcbf. 


% \begin{definition}[\newcbf]
%     Let $\mathcal{S}$ be as in \eqref{eq:safe_set_ro}.
%     % Let $\mathcal{S} \subset \R^n\times\R^p$ be the 0-superlevel set of a continuously differentiable function ${h:\R^n \times \R^p \to \R}$ with 0 a regular value. 
%     The function $h$ is a \newcbf for (\ref{eq:full_system}) with parameter function $\zeta: \R^n \times \R^p \times \R^m  \to \R_{>0}$ if there exists $\alpha>0$ such that for all $\widehat{\bs{\rho}} \in \R^p$ 
%     %and all $\mb{x} \in \R^n$
%     :
%     %$(x, \widehat{x}_\textrm{obs}) \in \mathcal{S}$:
%     \begin{align}
%         \sup_{\mb{v}\in \R^l} L_\mb{f}h(\mb{x}, \widehat{\bs{\rho}}) + L_\mb{g}h(\mb{x},  \widehat{\bs{\rho}}) \mb{v} \geq  - \alpha h(\mb{x},  \widehat{\bs{\rho}}) + \zeta ( \mb{x}, \widehat{\bs{\rho}}, \mb{v})   \label{eq:MRCBF-constraint}
%     \end{align}
%     % \begin{align}
%     %     \sup_{v\in \R^k} L_fh(x, \widehat{x}_\textup{obs}) + L_gh(x, \widehat{x}_\textup{obs}) v  - \sigma \Vert L_gh \Vert^2 - \epsilon(\mathcal{L}_{L_fh} + \mathcal{L}_{\alpha h } + \mathcal{L}_{\sigma \Vert L_gh \Vert^2} + \mathcal{L}_{L_gh} \Vert  v \Vert ) \geq - \alpha h(x, \widehat{x}_\textup{obs}) \label{eq:MRCBF-constraint}
%     % \end{align}
%     %where $\epsilon\geq \Vert \bs{\rho} - \widehat{x}_\textrm{obs} \Vert  $.% and $\mathcal{L}$ represents the Lipschitz constant of the subscripted functions. 
% \end{definition}
% % As presented in the Appendix \ref{apdx:thm_proof}, satisfying this constraint guarantees that \eqref{eq:desired_velocity_ISSf} holds even if $\bs{\rho}$ is not known directly. 
% By correctly choosing the function $\zeta$, this allows us to consider measurement uncertainty in addition to the tracking error and disturbance. This is summarized in the following theorem for which a proof can be found in Appendix \ref{apdx:thm_proof}.

% \begin{theorem} \label{thm:all_uncertainties}
% Consider system (\ref{eq:full_system}), $\delta$, $\alpha, \sigma$ as in Theorem \ref{thm:issf-cbf}. If $\mb{v}$ satisfies \eqref{eq:MRCBF-constraint} with parameter function 
% \begin{equation}
%     \zeta(\mb{x}, \widehat{\bs{\rho}}, \mb{v}) = \sigma \Vert L_\mb{g}h(\mb{x}, \widehat{\bs{\rho}}) \Vert^2 + a + b  \Vert \mb{v} \Vert\label{eq:param_func}
% \end{equation}
% where $ a \geq  \epsilon(\mathcal{L}_{L_\mb{f}h} + \mathcal{L}_{a h} + \mathcal{L}_{b \Vert L_\mb{g}h \Vert^2}) $, $ b \geq  \epsilon\mathcal{L}_{L_\mb{g}h} $, and $\mathcal{L}$ represents the Lipschitz constant of the subscripted functions, then $\mathcal{C}$ as defined in \eqref{eq:safe_set} is ISSf for system \eqref{eq:full_system}.
% \end{theorem}







% Theorem \ref{thm:all_uncertainties} accounts for the disturbance $\mb{d}$, the measurement uncertainty in  $\widehat{\bs{\rho}}$, and the reduced-order structure of (\ref{eq:full_system}) and states that any input that satisfies the \eqref{eq:MRCBF-constraint} will render $\mathcal{S}_e $ ISSf.
% However, the variables $a, b, c, d >0$ are all either user defined parameters or bounds which may be difficult to ascertain. Additionally, although values of these parameters exist to guarantee safety (assuming feasibility of the constraint), such values may be highly conservative and lead to undesirable behavior. The parametric nature of the \newcbf thus provides a nice structure for which \newpbl can be deployed to determine the user-preferred balance of performance with safety. 

==> drafts.tex <==
\section{Preliminaries}
Consider the control-affine system: 
\begin{align}
    \dot \x = \f (\x) + \g(\x) (\u + \mathbf{d}) \label{eq:dyn}
\end{align}
where $\x \in \R^n$, $u \in \R^m $, and $\f: \R^n \to \R^n$ and $\g : \R^n \to \R^{n\times m}$ are locally Lipschitz continuous.  



\begin{definition}[Control Lyapunov Function (CLF)]
A continuously differentiable function $V:\R^n \to \R_{\geq 0 }$ is a Control Lyapunov Funciton (CLF) for \eqref{eq:dyn} if there exists $c, k_1, k_2, \lambda \in \R_{>0}$ such that $\forall x \in \R^n $: 
\begin{align}
    k_1 \leq \Vert \x\Vert^c \leq V(\x) \leq k_2 \Vert \x \Vert^c \\
    \inf_{\u \in \R^m} \dot V(\x, \u)\geq - \lambda V(\x) 
\end{align}
\end{definition}


\begin{definition}[Input-to-State Stability (ISS)]
The system \eqref{eq:dyn} is Input-to-State Stable for $d: \R_{\geq 0 }\to \R^m $ if there exists $\beta\in \mathcal{KL}$ and $\iota \in \mathcal{K}$ such that: 
\begin{align}
    \Vert \x(t) \Vert \leq \beta(\Vert \x_0 \Vert, t) + \iota (\Vert \mathbf{d} \Vert_\infty),  \quad \forall \x_0 \in \R^ns, \;\; \forall t\geq 0 
\end{align}
\end{definition}

\subsection{Safety via Control Barrier Functions}


\subsection{Reduced-Order CBFs}
We consider a system \eqref{eq:dyn} safe if its state $\x $ stays within a safe set $\mathcal{C}\subset \R^n$ for all time. 
We define the safe set as the zero-superlevel set of a continuously differentiable function $h: \R^n \to \R $ with 0 a regular value. 

\begin{align}
    \mathcal{C} = \{ \x \in \R^n : h(\x) \geq 0  \}  & \partial \mathcal{C} = \{ \x \in \R^n : h(\x) = 0 \} & \textrm{Int}(\mathcal{C})  = \{ \x \in \R^n : h(\x) > 0  \} 
\end{align}

\begin{definition}[Safety]
The system is safe w.r.t $\mathcal{C}$ if $\mathcal{C}$ is forward invariant under \eqref{eq:dyn}, that is, $\x(0) \in \mathcal{C} \implies \x(t) \in \mathcal{C}, \forall t \geq 0  $. 
\end{definition}


\begin{definition}[Control Barrier Function (CBF)]
A continuously differentiable function $h: \R^n \to \R$ with 0 a regular value is a control barrier function (CBF) for \eqref{eq:dyn} if there exists $\alpha \in \R_{> 0}$ such that $\forall \x \in \mathcal{C}: $ 
\begin{align}
    \sup_{u\in\R^m} \underbrace{\dot h(\x, \u)}_{\frac{\partial h}{\partial \x } \big(\f(\x) + \g(\x)\u\big)} \geq -\alpha h(\x) 
\end{align}
\end{definition}

\begin{theorem}[\cite{ames2019control}] \label{thm:CBF}
If $h$ is a CBF for \eqref{eq:dyn}, then any locally Lipschitz continuous controller $\k: \R^n \to \R^m $ satisfying 
\begin{align}
    \dot h(\x, \k(\x)) \geq -\alpha h(\x)
\end{align}
$\forall \x \in \mathcal{C}$ renders \eqref{eq:dyn} safe w.r.t. $\mathcal{C}$.
\end{theorem}

Theorem \ref{thm:CBF} can be used to synthesize safe controllers. For example, given a desired, but not necessarily safe controller $\k_d(t)$, the safe CBF-QP controller can be defined as:  
\begin{align} \label{eq:CBF-QP} \tag{CBF-QP}
    \k_\textrm{cbf}(\x) =   \argmin_{\u\in\R^m} & \Vert \u - \k_d(t)\Vert^2\\
     \textrm{s.t. } & \dot h(\x,\u) \geq -\alpha h(\x) \nonumber
\end{align}



\subsection{Tunable ISSf}

\begin{definition}[Tunable ISSf (TISSf) \cite{alan2021safe}]
    Let $\mathcal{C} \subset \R^n $ be the 0-superlevel set of a continuously differentiably function $h: \R^n \to \R$ with 0 a regular value. Then $h$ is a tunable ISSf-CBF for the disturbed system \eqref{eq:dyn} if there exists $\alpha \in \mathcal{K}_{\infty, e}$ and a differentiable function $\epsilon: \R \to \R_{>0} $ such that for all $\x \in \R^n $" 
    \begin{equation}
        \sup_{\u \in \R^m } [L_\f h(\x) + L_\g h(\x) \u ] > -\alpha (h(\x)) + \frac{\Vert L_\g h(\x) \Vert^2 }{\epsilon(h(\x))  }
    \end{equation}
\end{definition}
% As outlined in \cite{grizzle2001asymptotically}, biepedal walking can described using a hydrid dynamical system with discrete transitions between continuous dynamics in different domains. The continuous dynamics are given by the affine control system: 

% \begin{align}
%     \dot \x = \f_v(\x)  + \g_v(\x) \u 
% \end{align}
% where $\x \in \R^n$ is the system state, $\u \in R^m $ are the inputs, $v \in \N_{\geq 0 }$ is the domain index, and $\f_v: \R^n \to \R^n $ and $\g_v: \R^n \to \R^m $ are locally Lipschitz functions on $\R^n $ for each $v$. The discrete transition between domains $v$ can be described as: 
% \begin{align}
%     \x^+ = \Delta_{v \to v+1 }(\x^-)
% \end{align}
% where the superscripts $^-$ and $^+$ stand for the instants before and after the trajectory respectively.

% Consider the projection function $\rho: \R^n \to \R^2$ that maps from to the robot state to the global position $\q \in \R^2$ where $\q \triangleq (x,y)$ the forward and lateral positoin.


\section{Uncertainties}
\subsection{Model Uncertainty}
\begin{assumption}[Low Level Tracking]
We assume that the low level controller provides (exponential?) ISS tracking. 
HLIP $\implies$ ISS 
\end{assumption}


Using the controller outlined in \cite{xiong20213d}, this assumption is justified by the tracking seen in \ref{fig:ISS_pic}


\subsection{Measurement Uncertainty}
\subsection{}


\begin{figure}[h!]
    \centering
    \includegraphics[width=6cm,height=10cm]{Figures/20211029_184621.jpg}
    \caption{Obviously there exists an ISS-CLF for Cassie, is depicted by the following plot. Real data on Cassie, recreated on the whiteboard for ease of visualization.}
    \label{fig:ISS_pic}
\end{figure}


\begin{proposition}
ISS-CLF tracking $\implies $ reduced-order ISSf. 
Given:
\begin{align}
    h_V(q,\dot e) = - V(q, \dot e) + \alpha_e h(q)
\end{align}
$\alpha_e \geq (\lambda - \alpha) k_1/C_h$, $C_h \geq \Vert \nabla h \Vert $, $k_1 \Vert \x \Vert^2 \leq V(\x) $. 
\end{proposition}
\begin{proof}
\begin{align}
    \dot h_V(q, \dot e, \dot q, \ddot q, u )  & = - \dot V(q, \dot e, \dot q , \ddot q , u ) + \alpha_e \nabla h(q)\dot q \\
    & \geq \lambda V(q, \dot e) - \frac{\partial V}{\partial \x }\g(\x)d(t) +  \alpha_e \nabla h (q)\dot q_s + \alpha_e \nabla h(q) \dot e \\
    & \geq (\lambda  - \alpha_e ) k_1 \Vert \dot e \Vert  - \alpha_e C_h \Vert \dot e \Vert - \alpha h_v  - \frac{\partial V}{\partial \x }\g(\x)d(t)\\
    & \geq - \alpha h_v - k_4 \Vert \dot e \Vert \Vert \g(\x) d(t) \Vert _\infty 
\end{align}
Following Tamas's proof \cite{molnar2021model}. So $h_V$ is ISSf. 
\end{proof}


Measurement uncertainty. Assume that the error enters because of perception error and thus through the position state $q$ and nowhere else. 

\subsection{Measurement Uncertainty to ISSf}
\begin{align}
    \nabla h(q)\dot q_s + \alpha h(q)  & = \nabla h(\widehat{q}) \dot q_s  + \alpha h(\widehat{q}) + \left( \nabla h(q) - \nabla h(\widehat{q}) \right) \dot q_s + \alpha (h(q) - \alpha h(\widehat{q}) ) \\
    & \geq \underbrace{\nabla h(\widehat{q}) \dot q_s + \alpha h (\widehat{q})}_{\geq 0 \textrm{, by choice of controller}}  - \Vert q - \widehat{q }\Vert (\mathcal{L}_{\alpha\circ h} + \mathcal{L}_{\nabla h } \Vert \dot q_s \Vert ) \\
    &\geq - \Vert q - \widehat{q }\Vert (\mathcal{L}_{\alpha\circ h} + \mathcal{L}_{\nabla h } \Vert \dot q_s \Vert )\\
    \nabla h(q)\dot q_s & \geq - \alpha h(q) - \Vert q - \widehat{q }\Vert (\mathcal{L}_{\alpha\circ h} + \mathcal{L}_{\nabla h } \Vert \dot q_s \Vert )
\end{align}

Assuming that the $V$ and $\dot V $ are not functions of $q$ which they should be because the low level controller should be agnostic to the global state, then the ISSf gets converted to: 
\begin{align}
    \dot h_v \geq - \alpha h_v - k_4 \Vert \dot e \Vert \Vert \g(\x) d(t) \Vert_\infty - \Vert q - \widehat{q} \Vert (\mathcal{L}_{\alpha\circ h } + \mathcal{L}_{\nabla h} \Vert \dot q_s\Vert) 
\end{align}
which is now a function of the desired input $\dot q_s $. These could be our parameters, since $k_4$ and $d(t) $ are unknown and $\mathcal{L}_{\alpha \circ h }$ and $\mathcal{L}_{\nabla h } \Vert \dot q_s \Vert $ are going to be really conservative.

The tuning parameters then seem to be
\begin{enumerate}
    \item the decay rate $\alpha$
    \item a constant ISSf term $k_4\Vert \dot e \Vert \Vert \g d \Vert  + \Vert q - \widehat{q} \Vert (\mathcal{L}_{\alpha \circ h}) $
    \item and an input bound term  $ \Vert q - \widehat{q} \Vert (\mathcal{L}_{\nabla h }\Vert \dot q_s\Vert ) $
\end{enumerate}
